Neighborly and almost neighborly configurations, and their duals

This thesis presents new applications of Gale duality to the study of polytopes, point configurations and oriented matroids with extremal combinatorial properties. The first part of the thesis explores construction techniques for neighborly polytopes and oriented matroids. First, we provide a new interpretation of Shemer's classical Sewing Construction for neighborly polytopes in terms of lexicographic extensions of oriented matroids. This allows us to provide a simplified proof and to generalize it to oriented matroids in two ways: the Extended Sewing Construction and the Gale Sewing Construction. Estimating the number of polytopes constructed with the later, we can provide new lower bounds for the number of combinatorial types of neighborly polytopes that even improve the current best bounds for the number of polytopes. The combination of both new techniques also allows us to construct many non-realizable neighborly oriented matroids. The degree of a point configuration is the maximal codimension of its interior faces. The second part of the thesis presents various results on the combinatorial structure of point configurations whose degree is small compared to their dimension; specifically, those whose degree is smaller than [(d+1)/2], the degree of neighborly polytopes. The study of this problem comes motivated by Ehrhart theory, where a notion equivalent to the degree - for lattice polytopes - has been widely studied during the last years. In addition, the study of the degree is also related to the Generalized Lower Bound Theorem for simplicial polytopes, with Cayley polytopes and with Tverberg theory. Among other results, we present a complete combinatorial classification for point configurations of degree 1. Moreover, we show combinatorial restrictions for configurations of small degree in terms of the novel concepts of weak Cayley configurations and codegree decompositions.

==> degree/degree.tex <==



==> neighborly/neighborly.tex <==

% \chapter{Many neighborly polytopes}


% \chapter{Balanced and Neighborly Oriented Matroids}
% \chapter{Preliminaries}





% \thispagestyle{empty}
% \chapter{The sewing construction}\label{ch:shemer}
% % \subsection{The sewing construction}
% 
% This section is devoted to explaining the sewing construction, introduced by Shemer in~\cite{Shemer1982}, that allows to construct an infinite class of neighborly polytopes.
% Even if Shemer described the sewing construction in terms of Gr\"unbaum's \emph{beneath-beyond} technique, it is in fact a lexicographic extension, and we will explain it in these terms. In this section, we use the letter $\cP$ for oriented matroids to reinforce the idea that all the following results translate directly to polytopes.
% % \subsection{Sewing through a flag}
% 
% Let $\cP$ be an acyclic oriented matroid and let $F$ be a facet of $\cP$. That is, there exists a cocircuit $C_F$ of $\cP$ such that $C_F(e)=0$ if $e\in F$ and $C_F(e)=+$ otherwise. Let $p$ be a single element extension of $\cP$ with signature $\gs_p$. We say that $p$ is 
% \defn{beneath}~$F$ if $\gs_p(C_F)=+$, that $p$ is \defn{beyond}~$F$ when $\gs_p(C_F)=-$, and that $p$ is \defn{on} $F$ if $\gs_p(C_F)=0$.
% We say that an extension $p$ of $\cP$ lies \defn{exactly beyond} a set of facets $\fF$ if it lies beyond all facets in $\fF$ and beneath all facets not in $\fF$.
% 
% 
% It is enough to know the signature of $p$ on the facet cocircuits of $\cP$ to tell the whole face lattice of $\cP\cup p$.
% 
% A \emph{flag} of an acyclic oriented matroid $\cP$ is a strictly increasing sequence of proper %\ojo{proper?} 
% faces $T_1\subset T_2 \subset \dots \subset T_k$. Given a flag $\cT=\{T_j\}_{j=1}^k$ of $\cP$, let $\cF_j$ be the set of facets of $\cP$ that contain $T_j$, and let $\fF(\cT):=\cF_1\setminus(\cF_2\setminus(\dots\setminus\cF_k)\dots)$; that is
% \begin{equation*}
% \fF(\cT)= 
% \begin{cases} (\cF_1\setminus\cF_2) \cup (\cF_3\setminus\cF_4)\cup \dots \cup (\cF_{k-1}\setminus\cF_k)& \text{if $k$ is even,}
% \\
% (\cF_1\setminus\cF_2) \cup (\cF_3\setminus\cF_4)\cup \dots \cup \cF_k &\text{if $k$ is odd.}
% \end{cases}
% \end{equation*}
% 
% %We say that $y\in \RR^d$ lies \defn{exactly beyond} $\fF$ if it lies beyond all facets in $\fF$ and beneath all facets in $\cF\setminus\fF$. Given a facet $F\in \cF$ and a point $x$ outside $\cP$, we say that $x$ is \defn{beneath} $F$ if $x$ and $\cP$ are at the same halfspace defined by $\aff{F}$. We say that $x$ is \defn{beyond} $F$ when $x$ and $\cP$ are separated by the hyperplane $\aff F$.
% 
% Given a polytope $P$ with a flag $\cT=T_1\subset T_2 \subset \dots \subset T_k$, Shemer proved that there always exists an extension exactly beyond $\fF(\cT)$, via the sewing construction. We will show that there is a lexicographic extension that realizes the desired signature.
% 
% \begin{definition}[Sewing onto a flag]\label{def:sewing}
% Let $\cT=\{T_j\}_{j=1}^k$ be a flag of an acyclic matroid $\cP$. We extend it with $T_{k+1}=\cP$ and define $U_i=T_i\setminus T_{i-1}$. 
% We say that $p$ is \emph{sewn} onto $\cP$ through $\cT$, if $p$ is a lexicographic extension 
% \begin{displaymath}p=[T_1^+,U_2^-,U_3^+,\dots,U_{k+1}^{(-1)^{k}}],\end{displaymath}
% where these sets represent their elements in any order. 
% 
% % That is, if $a_1, \dots, a_{n}$ are the points in $T_{k+1}$, sorted such that if $a_i$ belongs to a $T_s$ and $a_j$ does not, then $i<j$, then
% %  $p$ is a lexicographic extension $p=[a_1^{s_1},a_2^{s_2},\dots,a_{n}^{s_{n}}]$, where $s_j$ is $+$ if the smallest $i$ such that $x_j\in T_i$ is odd, and $-$ otherwise.
% That is, $p$ is a lexicographic extension $p=[a_1^{s_1},a_2^{s_2},\dots,a_{n}^{s_{n}}]$ where $a_1, \dots, a_{n}$ are the points in $T_{k+1}$, sorted such that if $a_i$ belongs to a $T_s$ and $a_j$ does not then $i<j$, and where $s_j$ is $+$ if the smallest $i$ such that $x_j\in T_i$ is odd, and $-$ otherwise.
% 
% 
% We use the notation $\cP[\cT]$ to designate the extension $\cP\cup p$ when $p$ is sewn onto~$\cP$ through $\cT$.
% \end{definition}
% 
% In terms of oriented matroids, the definition of $\cP[\cT]$ is ambiguous, since it can represent different oriented matroids. However, the following proposition shows that all the extensions $\cP[\cT]$ have the same face lattice. Moreover, because of rigidity, this implies that there is no ambiguity when $\cP[\cT]$ is neighborly of odd rank.
% 
% \begin{proposition}\label{prop:exactlybeyondle}
% Let $\cT=\{T_j\}_{j=1}^k$ be a flag of an acyclic oriented matroid $\cP$, and let $\fF(\cT):=\cF_1\setminus(\cF_2\setminus(\dots\setminus\cF_k)\dots)$. If $p$ is the lexicographic extension $\cP\cup p=\cP[\cT]$, then $p$ lies exactly beyond $\fF$.
% \end{proposition}
% \begin{proof}
% % Let $T_{k+1}$ be a subsimplex of $\cP$ that contains $T_k$. 
% % Let $x_1,\dots, x_{d+1}$ be the points in $T_{k+1}$, sorted such that if $x_i$ belongs to a $T_s$ and $x_j$ does not, then $i<j$. And let
% %  $p$ be the lexicographic extension $[x_1^{s_1},x_2^{s_2},\dots,x_{d+1}^{s_{d+1}}]$, where $s_j$ is $+$ if the smallest $i$ such that $x_j\in T_i$ is odd, and $-$ otherwise.
% Let $p$ be the lexicographic extension $[a_1^{s_1},a_2^{s_2},\dots,a_{d+1}^{s_{d+1}}]$ from Definition~\ref{def:sewing}.
% We have to see that $p$ lies beneath any facet in $\cF_{2j}\setminus\cF_{2j+1}$ and beyond any facet in $\cF_{2j-1}\setminus\cF_{2j}$.
% 
% If $C$ is a cocircuit representing a facet $F$ in $\cF_{j}\setminus\cF_{j+1}$, then the first $a_i$ with $C(a_i)\neq 0$ belongs to $T_{j+1}$.
% If $j$ is even then $s_i=+$ and hence $p$ is beneath $F$. If $j$ is odd then $s_i=-$ and $p$ is beyond $F$. 
% \end{proof}
% 
% The sewing construction starts with a neighborly oriented matroid $\cP$ of rank~$d$ with $n$ elements and gives a neighborly oriented matroid $\tilde \cP$ of rank $d$ with $n+1$ elements, provided that $\cP$ has a $\emph{universal flag}$.
% 
% \begin{definition}
% Let $\cP$ be a uniform acyclic oriented matroid on $E$ of rank $d$, and let $m=\ffloor{d-1}{2}$.
% \begin{enumerate}[(i)]
% %  \item $F\subseteq E$ is a \emph{face} of $\cP$ if there is a covector $C$ of $\cP$ with $C^+=E\setminus F$ and $C^-=\emptyset$.
%  \item A face $F$ of $\cP$ is a \emph{universal face} if the contraction $\cP/F$ is neighborly.
% %  \item A \emph{flag} of $\cP$ is a strictly increasing sequence of faces $T_1\subset T_2 \subset \dots \subset T_k$. %\ojo{$T_1\neq \emptyset$ ?}
%  \item A flag $\cT$ of $\cP$ is a \emph{universal flag} if $\cT=\{T_j\}_{j=1}^m$ where each $T_j$ is a universal face with $2j$ vertices.
% \end{enumerate}
% \end{definition}
% 
% The first example of neighborly polytopes with universal flags are cyclic polytopes (see {\cite[Theorem 3.4]{Shemer1982}}).
% 
% \begin{example}\label{ex:universalflagsofcyclic}
% Let $\cyc{n}{2m}$ be a cyclic polytope of even dimension $2m$, with vertices $s_1,\dots,s_n$ labeled in cyclic order. Then $\{s_i,s_{i+1}\}$, $1\leq i<n$ and $\{s_1,s_{n}\}$ are universal edges of $\cyc{n}{2m}$.
% Moreover, $\cyc{n}{2m}/\{s_i,s_{i+1}\}\simeq \cyc{n-2}{2m-2}$ with the same cyclic order. 
% % Moreover, if $E_1,\dots,E_r$ are pairwise disjoint universal edges of $\cyc{n}{2m}$, then $E_1\cup \dots \cup E_r$ is a universal face of $\cyc{n}{2m}$.
% % This gives a large family of universal flags of $\cyc{n}{2m}$.
% % , $T_1\subset T_2 \subset \dots \subset T_m$, where every $T_i$ is of the form $\{s_j,s_{j+1},\dots, s_{j+2i-1}\}$ for a $1\leq j\leq n$ and subscripts modulo $n$.
% In particular this gives a large family of universal flags of $\cyc{n}{2m}$ formed by faces that are the union of a universal edge of $\cyc{n}{2m}$ with a (possibly empty) universal face of $\cyc{n-2}{2m-2}$.
% \end{example}
% % 
% % \begin{definition}[Sewing onto a flag]
% % Let $\cT=\{T_j\}_{j=1}^k$ be a flag of $\cP$. We extend it with $T_{k+1}=\cP$ and define $U_i=T_i\setminus T_{i-1}$. 
% % We say that $p$ is \emph{sewn} onto $\cP$ through $\cT$, if $p$ is a lexicographic extension 
% % \begin{displaymath}p=[T_1^+,U_2^-,U_3^+,\dots,U_{k+1}^{(-1)^{k}}],\end{displaymath}
% % where these sets represent their elements in any order. 
% % % 
% % % That is, if $x_1, \dots, x_{n}$ are the points in $T_{k+1}$, sorted such that if $x_i$ belongs to a $T_s$ and $x_j$ does not, then $i<j$, then
% % %  $p$ is a lexicographic extension $p=[x_1^{s_1},x_2^{s_2},\dots,x_{n}^{s_{n}}]$, where $s_j$ is $+$ if the smallest $i$ such that $x_j\in T_i$ is odd, and $-$ otherwise.
% % \end{definition}
% % 
% % We use the notation $\cP[\cT]$ to designate $\cP\cup p$ if $p$ is sewn onto $\cP$ through $\cT$.
% % 
% % % \begin{definition}
% % % 
% % % Let $\cT=\{T_j\}_{j=1}^k$ be a flag of a matroid polytope $\cP$ and let $T_{k+1}$ be a subsimplex of $\cP$ that contains $T_k$. Let $x_1, \dots, x_{d+1}$ be the points in $T_{k+1}$, sorted such that if $x_i$ belongs to a $T_s$ and $x_j$ does not, then $i<j$.
% % % 
% % % We say that $p$ is \emph{sewn} onto $\cP$ through $\cT$, if $p$ is a lexicographic extension $p=[x_1^{s_1},x_2^{s_2},\dots,x_{d+1}^{s_{d+1}}]$, where $s_j$ is $+$ if the smallest $i$ such that $x_j\in T_i$ is odd, and $-$ otherwise.
% % % 
% % % That is, if $U_i=T_i\setminus T_{i-1}$, then is the lexicographic extension on $[T_1^+,U_2^-,U_3^+,\dots,U_{k+1}^{(-1)^{k}}]$, where these sets represent their elements in any order. We will use the notation $\cP[\cT]$ to designate $\cP\cup p$.
% % % \end{definition}
% 
% 
% % \begin{lemma}\label{lem:quotientsofShemersewing}
% % Let $\cP$ be a uniform neighborly matroid of rank $d$ with a universal flag $\cT=\{T_j\}_{j=1}^m$, where $T_j=\{x_i,y_i\}_{i=1}^{j}$
% % and $m=\ffloor{d-1}{2}$. Let $p$ be sewn onto $\cP$ through $\cT$.
% % Then \begin{displaymath}\cP[\cT]/\{T_{i-1},x_{i},p\}\simeq\cP[\cT]/\{T_{i-1},y_{i},p\}\simeq (\cP/T_i)[\cT/T_i],\end{displaymath}
% % where $\cT/T_i=\{T_j/T_i\}_{j=i+1}^{m}$ and $T_j/T_i$ is the face of $\cP/T_i$ that represents $T_j$.
% % The first isomorphism sends $y_{i}$ to $x_{i}$ and the second sends $x_{i}$ to the sewn vertex. The rest of the isomorphisms are the natural mappings.
% % \end{lemma}
% % \begin{proof}
% % % A consequence of $\{x_1,y_1\}$ being a universal edge is that $x_1$ and $y_1$ are contravariant, which implies that $[x_1^+,y_1^+,\dots]$ and $[y_1^+,x_1^+,\dots]$ are the same lexicographic extensions. This proves the symmetric behavior of $x_i$ and $y_i$.
% % % The symmetric behavior of $x_i$ and $y_i$ is a consequence of $\{x_i,y_i\}$ being a universal edge in $\cP/T_{i-1}$, which implies that their order in the lexicographic extension $\cP[\cT]$ can be changed. 
% % % Since $\{x_i,y_i\}$ is a universal edge in $\cP/T_{i-1}$, they are contravariant and their order in the lexicographic extension $\cP[\cT]$ can be changed. This explains their symmetric behavior.
% % The 
% % % rest of the
% %  proof relies on using Proposition~\ref{prop:allquotientsofle} twice on the lexicographic extension $\cP[\cT]$,
% % % , that is $$\cP[\cT]=\cP[x_1^+,y_1^+,x_2^-,y_2^-,\dots,x_m^{(-1)^{m-1}},y_m^{(-1)^{m-1}},x_{m+1}^{(-1)^{m}},y_{m+1}^{(-1)^{m}}].$$
% % % It is easy to check that
% % and follows inductively from
% % % $$\cP[\cT]/\{T_{i-1}\}\simeq (\cP/T_{i-1})[\cT/T_{i-1}],$$
% % % and that $$ \cP[\cT]/\{p,x_1\}\simeq \cP[\cT]/\{p,y_1\}\simeq \cP/T_1[\cT/T_1].$$ 
% % % \begin{displaymath}\cP[\cT]/T_{i-1}\simeq (\cP/T_{i-1})[\cT/T_{i-1}]\quad\text{ and }\quad\cP[\cT]/\{p,x_1\}\simeq \cP[\cT]/\{p,y_1\}\simeq \cP/T_1[\cT/T_1].\end{displaymath}
% % \(\cP[\cT]/\{p,x_1\}\simeq \cP[\cT]/\{p,y_1\}\simeq \cP/T_1[\cT/T_1].\)
% % \end{proof}
% 
% With these notions, we are ready to present Shemer's Sewing Theorem~\cite[Theorem 4.6]{Shemer1982}.
% \begin{theorem}[The Sewing Theorem]\label{thm:shemersewing}
% Let $P$ be a neighborly polytope of dimension $2m$ with a universal flag $\cT=\{T_j\}_{j=1}^m$, where $T_j=\{x_i,y_i\}_{i=1}^{j}$.
% Let $\tilde P=P[\cT]$, with $p$ sewn onto $P$ through~$\cT$.
%  Then,
% \begin{enumerate}
% \item\label{it:newisneigh} $\tilde P$ is a neighborly polytope with vertices $\verts (\tilde P)=\verts (P)\cup \{p\}$.
% \item\label{it:newunifaces} For all $1\leq j \leq m$, $T_{j-1}\cup\{x_j,p\}$ and $T_{j-1}\cup\{y_j,p\}$ are universal faces of $\tilde P$. If moreover $j$ is even, then $T_j$ is also a universal face of $\tilde P$.
% \end{enumerate} 
% \end{theorem}
% 
% Combining Example~\ref{ex:universalflagsofcyclic} and Theorem~\ref{thm:shemersewing}, one can obtain a large family of neighborly polytopes: starting with an even-dimensional cyclic polytope and one of its universal flags, sew a new vertex onto it and obtain a new neighborly polytope (point~\ref{it:newisneigh} of Theorem~\ref{thm:shemersewing}) with new universal flags (from point~\ref{it:newunifaces} of Theorem~\ref{thm:shemersewing}). Since the new polytope has universal flags, one can keep sewing again. This method generates a family of neighborly polytopes \emph{$\cS$}, that we call \emph{totally sewn} polytopes\footnote{Shemer's concept of totally sewn polytopes is slightly different, because we only admit those flags that come from Theorem~\ref{thm:shemersewing}.}.
% 
% % 
% % With these tools, we can prove our version of the sewing theorem \cite[Theorem 4.6]{Shemer1982}, extended to neighborly matroids of any rank.
% % 
% % \begin{theorem}[The Sewing Theorem]\label{thm:shemersewing}
% % Let $\cP$ be a uniform neighborly matroid of rank $d$ with a universal flag $\cT=\{T_j\}_{j=1}^m$, where $T_j=\{x_i,y_i\}_{i=1}^{j}$
% % %\ojo{, $n\geq d+3$ (cal?)} 
% % and $m=\ffloor{d-1}{2}$.
% % %\ojo{$m=\ffloor{d}{2}\geq 2$  cal?}. 
% % %Let $\tilde \cP= \cP[x_1^+,y_1^+,x_2^-,y_2^-,\dots,x_m^{(-1)^{m+1}},y_m^{(-1)^{m+1}},*]$. 
% % Let $\tilde \cP=\cP[\cT]$, with $p$ sewn onto $\cP$ through~$\cT$.
% % % Then,
% % \begin{enumerate}
% % \item\label{it:newisneigh} $\tilde \cP$ is a uniform neighborly matroid of rank $d$.
% % \item\label{it:newunifaces} Let $\tilde T_j=[T_{j-1},z_j,p]$, where $z_j\in \{x_{j},y_{j}\}$ and $1\leq j \leq m$. Then $\tilde T_j$ is a universal face of $\tilde \cP$.
% % \end{enumerate} 
% % \end{theorem}
% % 
% % \begin{proof}
% % 
% % $\tilde \cP=\cP \cup p$ is the lexicographic extension 
% % \begin{displaymath}\tilde \cP= \cP\left[x_1^+,\;y_1^+,\;x_2^-,\;y_2^-,\;\dots,\;x_m^{(-1)^{m-1}},\;y_m^{(-1)^{m-1}},\;x_{m+1}^{(-1)^{m}},\;y_{m+1}^{(-1)^{m}}\right],\end{displaymath} 
% % where $x_{m+1}$ and $y_{m+1}$ are any two elements of $\cP$ not in $T_m$.
% % We check that $\tilde \cP$ is neighborly by checking that $\tilde \cP^*$ is balanced, \ie we check that every circuit $X$ of $\tilde \cP$ is halving:
% % % For this, we will associate each circuit of $\tilde \cP$ with some other circuit with the same discrepancy and that we already know that is halving.
% % \begin{enumerate}
% %  \item If $X(p)=0$, then $X$ is halving, since it is a circuit of $\cP$, and $\cP$ is neighborly.
% %  \item If $X(p)\neq 0$ and $X({x_1})=0$, we will see that there is a circuit $X'$ of $\tilde \cP$ with $X'(p)=0$ and $X'(x_1)\neq 0$, such that $|X^+|=|X'^+|$ and $|X^-|=|X'^-|$. Hence $X$ is halving by the previous point.
% % 
% % Let $X'\in \ci(\tilde \cP)$ be the circuit with support $\underline X'=\underline X \setminus p \cup x_1$ and such that $X'({x_1})=X(p)$. We will see that $X'({e})=X(e)$ for all $e\in E$.
% % Let $e\in \underline{X}\setminus p$, and let $C$ be the cocircuit of $\tilde\cP$ with $\underline C=E\setminus(\underline{X}\setminus p\setminus e)$. That makes $\underline C\cap \underline X=\{e,p\}$. Using that $p$ and $x_1$ are contravariant, and by circuit-cocircuit orthogonality, 
% % \begin{displaymath}X(p)X(e)=-C(p)C(e)=-C({x_1})C(e).\end{displaymath}
% % But $\underline C\cap \underline X'=\{e,x_1\}$, and hence, again by orthogonality, \begin{displaymath}X'(x_1)X'(e)=-C({x_1})C(e).\end{displaymath}
% % The conclusion now follows from $X'({x_1})=X(p)$. 
% % % 
% % % 
% % % Let $B=E\setminus(\underline{X}\setminus p)$, let $e\in E$ be an element that does not belong to $B$, and let $C$ be the cocircuit of $\tilde\cP$ with $\underline C=B\cup e$. Using that $p$ and $x_1$ are contravariant, and by orthogonality, 
% % % $$X(p)X(e)=-C(p)C(e)=-C({x_1})C(e).$$
% % % But $\underline C\cap \underline X'=\{e,x_1\}$, and hence, again by orthogonality, $$X'(x_1)X'(e)=-C({x_1})C(e).$$
% % \item If $X(p)\neq 0$ and $X({x_1})\neq 0$, since $p$ and $x_1$ are contravariant, $X(p)=-X({x_1})$. Observe that the rest of the values of $X$ correspond to a circuit of $\tilde \cP/\{p,x_1\}$. If $\tilde \cP/\{p,x_1\}$ is balanced, we are done.
% % 
% % By Lemma~\ref{lem:quotientsofShemersewing}, $\tilde \cP/\{p,x_1\}\simeq \cP/T_1[\cT/T_1]$. Since $\{x_1,y_1\}$ was a universal edge, $\cP/T_1$ is a neighborly matroid and $\cT/T_1$ is a universal flag. Then the result follows by induction on $d$. Observe for the base case that all acyclic universal matroids of rank $1$ or $2$ are neighborly.
% % \end{enumerate}
% % 
% % % It is clear that the circuits $X$ of $\tilde \cP$ with $X(p)=0$ are halving, since they are circuits of $\cP$.
% % 
% % % Circuits $X$ of $\tilde \cP$ with $X(p)\neq 0$ and $X({x_1})=0$ will correspond to circuits $X'$ of $\tilde \cP$ with $X(p)= 0$ and $X({x_1})\neq 0$, and hence they are also halving.
% % % 
% % % To see it, fix a circuit $X\in \ci(\tilde \cP)$ with $X(p)\neq 0$ and $X({x_1})=0$ and let $X'\in \ci(\tilde \cP)$ be the circuit with support $\underline X'=\underline X \setminus p \cup x$ and such that $X'({x_1})=X(p)$. We will see that $X'({e})=X(e)$ for all $e\in E$.
% % % 
% % % Let $B=E\setminus(\underline{X}\setminus p)$, let $e\in E$ be an element that does not belong to $B$, and let $C$ be the cocircuit of $\tilde\cP$ with $\underline C=B\cup e$. Using that $p$ and $x_1$ are contravariant, and by orthogonality, $$X(p)X(x)=-C(p)C(e)=-C({x_1})C(e).$$
% % % But $\underline C\cap \underline X'=\{e,x_1\}$, and hence, again by orthogonality, $$X'(p)X'(x)=-C({x_1})C(e).$$
% % % 
% % % Finally, for the circuits with $X(p)\neq 0$ and $X({x_1})\neq 0$, since they are contravariant, $X(p)=-X({x_1})$. Observe that the rest of values of $X$ correspond to circuits of $\tilde \cP/\{p,x_1\}$. If all those circuits are halving, we are done.
% % % 
% % % By Lemma~\ref{lem:quotientsofShemersewing}, $\tilde \cP/\{p,x_1\}\simeq \cP/T_1[\cT/T_1]$. Since $\{x_1,y_1\}$ was a universal edge, $\cP/\{T_1\}$ is a neighborly matroid and $\cT/T_1$ is a universal flag. Then the result follows by induction. Observe for the base case, that all acyclic universal matroids of rank $1$ or $2$ are neighborly.
% % 
% % 
% % The second claim of the theorem is also a direct consequence of Lemma~\ref{lem:quotientsofShemersewing}.
% % % This last proof by induction gives also directly claim~\eqref{it:newunifaces}. 
% % \end{proof}
% 
% 
% In Theorem~\ref{thm:extshemersewing} we generalize Theorem~\ref{thm:shemersewing} to neighborly oriented matroids. Our formulation, like \cite[Theorem 2]{Bisztriczky2000}, does not depend on the parity of the rank. Moreover, it is extended to any flag that contains a universal subflag, as suggested in~\cite[Remark 7.4]{Shemer1982}. In order to prove it, we need a lemma.
% % 
% % \begin{lemma}\label{lem:quotientsofextShemersewing}
% % Let $\cP$ be a uniform matroid of rank $d$. Let $\cT'=\{T_j'\}_{j=1}^k$ be a flag of $\cP$ that contains a subflag $\cT=\{T_j\}_{j=1}^m$, where $T_j=\{x_i,y_i\}_{i=1}^{j}$ and $m=\ffloor{d-1}{2}$. Let $p$ be sewn onto $\cP$ through $\cT'$.
% % 
% % If neither $T_{i-1}\cup \{x_{i}\}$ nor $T_{i-1}\cup \{y_{i}\}$ belong to $\cT'$, then
% % \begin{equation}\label{eq:quoShemer1}\cP[\cT']/\{T_{i-1},x_{i},p\}\simeq\cP[\cT']/\{T_{i-1},y_{i},p\}\simeq (\cP/T_i)[\cT'/T_i].\end{equation}
% % 
% % If $T_{i-1}\cup \{x_{i}\}$ belongs to $\cT'$, then 
% % \begin{equation}\label{eq:quoShemer2}\cP[\cT']/\{T_{i-1},x_{i},p\}\simeq\cP[\cT']/\{T_{i-1},x_{i},y_{i}\}\simeq (\cP/T_i)[\cT'/T_i].\end{equation}
% % 
% % In \eqref{eq:quoShemer1} and \eqref{eq:quoShemer2}, we use the notation $\cT'/T_i=\{T_j'/T_i\}_{j=i+1}^{m}$ where $T_j'/T_i$ is the face of $\cP/T_i$ that represents $T_j'$.
% % 
% % The first isomorphism of \eqref{eq:quoShemer1} sends $y_{i}$ to $x_{i}$ and the second sends $x_{i}$ to the sewn vertex. The first isomorphism of \eqref{eq:quoShemer2} sends $y_{i}$ to $p$ and the second sends $p$ to the sewn vertex. The rest of the isomorphisms are the natural mappings.
% % \end{lemma}
% % \begin{proof}
% % Since \(\cP[\cT]/T_{i-1}\simeq (\cP/T_{i-1})[\cT/T_{i-1}]\), it is enough to prove the lemma for $i=1$. We use the notation $U_i=T_i'\setminus T_{i-1}'$.
% % 
% % If $T_1'=\{x_1,y_1\}$, then $\cP[\cT']=\cP[x_1^+,y_1^+,U_2^-,\dots]$. Using Proposition~\ref{prop:allquotientsofle} twice on the lexicographic extension $\cP[\cT']$ we get \(\cP[\cT]/\{p,x_1\}\simeq \cP[\cT]/\{p,y_1\}\simeq \cP/T_1[\cT/T_1].\)
% % 
% % And if $T_1'=\{x_1\}$ and $T_2'=\{x_1,y_1\}$, then $\cP[\cT']=\cP[x_1^+,y_1^-,U_3^+,\dots]$. Using Proposition~\ref{prop:allquotientsofle} twice on the lexicographic extension $\cP[\cT']$ we get \(\cP[\cT]/\{p,x_1\}\simeq \cP[\cT]/\{x_1,y_1\}\simeq \cP/T_1[\cT/T_1].\)
% % \end{proof}
% 
% We will use the notation $\cT'/T_i=\{T_j'/T_i\}_{j=i+1}^{m}$ where $T_j'/T_i$ is the face of $\cP/T_i$ that represents $T_j'$. 
% 
% \begin{lemma}\label{lem:quotientsofextShemersewing}
% Let $\cP$ be a uniform neighborly matroid of rank $d$. Let $\cT'=\{T_j'\}_{j=1}^k$ be a flag of $\cP$ that contains a universal subflag $\cT=\{T_j\}_{j=1}^m$,
%  where $m=\ffloor{d-1}{2}$ and $T_j=\{x_i,y_i\}_{i=1}^{j}$.
% %  where $T_j=\{x_i,y_i\}_{i=1}^{j}$ and $m=\ffloor{d-1}{2}$.
%  Let $p$ be sewn onto $\cP$ through $\cT'$. If $T_{i-1}\cup \{y_{i}\}$ does not belong to $\cT'$, then
% \begin{equation*}%\label{eq:quoShemer1}
% \cP[\cT']/\{T_{i-1},x_{i},p\}\simeq (\cP/T_i)[\cT'/T_i].\end{equation*}
% 
% The isomorphism sends $y_{i}$ to the sewn vertex and the remaining are the natural mappings.
% \end{lemma}
% % \begin{proof}
% % % Since \(\cP[\cT]/T_{i-1}\simeq (\cP/T_{i-1})[\cT/T_{i-1}]\), it is enough to prove the lemma for $i=1$. 
% % If $U_i=T_i'\setminus T_{i-1}'$, observe that by Proposition~\ref{prop:allquotientsofle}, $\cP[\cT']/T_{i-1}$ must be one of the extensions
% % \begin{equation*}
% % \cP[\cT']/T_{i-1} = 
% % \begin{cases} 
% % \cP/T_{i-1}[x_i^+,y_i^+,U_{i+1}^-,\dots],
% % \\
% % \cP/T_{i-1}[x_i^-,y_i^-,U_{i+1}^+,\dots],
% % \\
% % \cP/T_{i-1}[x_i^+,y_i^-,U_{i+1}^+,\dots],% \quad \text{ or }
% % \\
% % \cP/T_{i-1}[x_i^-,y_i^+,U_{i+1}^-,\dots].
% % \end{cases}
% % \end{equation*}
% % The first two cases being possible if $U_i=\{x_i,y_i\}$ and the second two cases being possible if $U_i=\{x_i\}$. Using Proposition~\ref{prop:allquotientsofle} twice on each of these lexicographic extensions we get \(\cP[\cT']/\{T_{i-1},x_{i},p\}\simeq (\cP/T_i)[\cT'/T_i]\).
% % \end{proof}
% \begin{proof}
% % Since \(\cP[\cT]/T_{i-1}\simeq (\cP/T_{i-1})[\cT/T_{i-1}]\), it is enough to prove the lemma for $i=1$. 
% % Observe that by Proposition~\ref{prop:allquotientsofle}, $\cP[\cT']/T_{i-1}$ must be one of the extensions
% By Proposition~\ref{prop:allquotientsofle}, the contraction $\cP[\cT']/T_{i-1}$ is a lexicographic extension of $\cP/T_{i-1}$ whose signature coincides with that of $[\cT']$ by removing the first $2(i-1)$ elements. Hence $\cP[\cT']/T_{i-1}$ must be one of the extensions
% \begin{equation*}
% \cP[\cT']/T_{i-1} = 
% \begin{cases} 
% \cP/T_{i-1}[x_i^+,y_i^+,x_{i+1}^-,\dots],
% \\
% \cP/T_{i-1}[x_i^-,y_i^-,x_{i+1}^+,\dots],
% \\
% \cP/T_{i-1}[x_i^+,y_i^-,x_{i+1}^+,\dots],% \quad \text{ or }
% \\
% \cP/T_{i-1}[x_i^-,y_i^+,x_{i+1}^-,\dots].
% \end{cases}
% \end{equation*}
% 
% If $T'_{j-1}$ is the face of $\cT'$ corresponding to $T_{i-1}$, and $U'_{j}=T'_{j}\setminus T'_{j-1}$, then the first two cases are possible when $U'_{j}=\{x_i,y_i\}$ and the last two cases are possible when $U'_{j}= \{x_i\}$.
% % The first two cases being possible if $\cT'=\dots\subset T_{i-1}\subset T_{i-1}\cup \{x_i,y_i\}\subset\dots$ and the last two cases being possible if $\cT'=\dots\subset T_{i-1}\subset T_{i-1}\cup \{x_i\}\subset T_{i-1}\cup \{x_i,y_i\}\subset\dots$. 
% We use Proposition~\ref{prop:allquotientsofle} twice on each of these (contracting successively	 $x_i$ and $p$) to get \(\cP[\cT']/\{T_{i-1},x_{i},p\}\simeq (\cP/\{T_{i-1},x_{i},y_i\})[x_{i+1}^+,\dots]=(\cP/T_i)[\cT'/T_i]\).
% \end{proof}
% 
% We can finally state and prove the Extended Sewing Theorem.
% % With these tools, we can prove a general version of the sewing theorem \cite[Theorem 4.6]{Shemer1982}. It is extended to neighborly matroids of any rank and to all flags that contain a universal flag.
% 
% \begin{theorem}[The Extended Sewing Theorem]\label{thm:extshemersewing}
% Let $\cP$ be a uniform neighborly oriented matroid of rank $d$ with a universal flag $\cT=\{T_j\}_{j=1}^m$, where $T_j=\{x_i,y_i\}_{i=1}^{j}$
% and $m=\ffloor{d-1}{2}$. Let $\cT'=\{T_j'\}_{j=1}^k$ be a flag of $\cP$ that contains $\cT$ as a subflag. Let $\tilde \cP=\cP[\cT']$, with $p$ sewn onto $\cP$ through~$\cT'$. Then % Then,
% % \begin{enumerate}
% % \item\label{it:newisneigh} 
% $\tilde \cP$ is a uniform neighborly matroid of rank $d$.
% % \item\label{it:newunifaces} Let $\tilde T_j=[T_{j-1},z_j,p]$, where $z_j\in \{x_{j},y_{j}\}$ and $1\leq j \leq m$. Then $\tilde T_j$ is a universal face of $\tilde \cP$.
% % \end{enumerate} 
% \end{theorem}
% \begin{proof}
% % Using the notation $U_i=T_i'\setminus T_{i-1}'$, then $\tilde \cP=\cP \cup p$ is either the lexicographic extension 
% % \(\tilde \cP= \cP\left[x_1^+,\;y_1^+,\;U_2^-,\;\dots,\right],\) or \(\tilde \cP= \cP\left[x_1^+,\;y_1^-,\;U_2^+,\;\dots,\right]\), depending on whether $T'_1=\{x_1,y_1\}$ or $T'_1=\{x_1\}$. 
% Depending on whether $T'_1=\{x_1,y_1\}$ or $T'_1=\{x_1\}$, the extension $\tilde \cP=\cP \cup p$ is either the lexicographic extension 
% \(\tilde \cP= \cP\left[x_1^+,y_1^+,\dots\right]\), or \(\tilde \cP= \cP\left[x_1^+,y_1^-,\dots\right]\). 
% 
% We check that $\tilde \cP$ is neighborly by checking that $\tilde \cP^*$ is balanced, \ie we check that every circuit $X$ of $\tilde \cP$ is halving:
% % For this, we will associate each circuit of $\tilde \cP$ with some other circuit with the same discrepancy and that we already know that is halving.
% \begin{enumerate}
%  \item If $X(p)=0$, then $X$ is halving, since it is a circuit of $\cP$, and $\cP$ is neighborly.
%  \item If $X(p)\neq 0$ and $X({x_1})=0$, we use that $p$ and $x_1$ are contravariant. By Lemma~\ref{lem:circinseparable}, if $X'\in \ci(\tilde \cP)$ is the circuit with $X'({x_1})=X(p)$ and support $\underline X'=\underline X \setminus p \cup x_1$, then $|X^+|=|X'^+|$ and $|X^-|=|X'^-|$. Since $X'(p)=0$% and $X'(x_1)\neq 0$
% , $X'$ is halving by the previous point. Hence so is $X$.
%  \item If $X(p)\neq 0$ and $X({x_1})\neq 0$, since $p$ and $x_1$ are contravariant, $X(p)=-X({x_1})$. Observe that the rest of the values of $X$ correspond to a circuit of $\tilde \cP/\{p,x_1\}$. If $\tilde \cP/\{p,x_1\}$ is balanced, we are done.
% 
% By Lemma~\ref{lem:quotientsofextShemersewing}, $\tilde \cP/\{p,x_1\}\simeq \cP/T_1[\cT'/T_1]$. Since $\{x_1,y_1\}$ was a universal edge, $\cP/T_1$ is a neighborly matroid and $\cT'/T_1$ is a flag that contains the universal flag $\cT/T_1$. Then the result follows by induction on $d$. Observe for the base case that all acyclic universal matroids of rank $1$ or $2$ are neighborly.
% \end{enumerate}
% % It is clear that the circuits $X$ of $\tilde \cP$ with $X(p)=0$ are halving, since they are circuits of $\cP$.
% % Circuits $X$ of $\tilde \cP$ with $X(p)\neq 0$ and $X({x_1})=0$ will correspond to circuits $X'$ of $\tilde \cP$ with $X(p)= 0$ and $X({x_1})\neq 0$, and hence they are also halving.
% % 
% % To see it, fix a circuit $X\in \ci(\tilde \cP)$ with $X(p)\neq 0$ and $X({x_1})=0$ and let $X'\in \ci(\tilde \cP)$ be the circuit with support $\underline X'=\underline X \setminus p \cup x$ and such that $X'({x_1})=X(p)$. We will see that $X'({e})=X(e)$ for all $e\in E$.
% % 
% % Let $B=E\setminus(\underline{X}\setminus p)$, let $e\in E$ be an element that does not belong to $B$, and let $C$ be the cocircuit of $\tilde\cP$ with $\underline C=B\cup e$. Using that $p$ and $x_1$ are contravariant, and by orthogonality, $$X(p)X(x)=-C(p)C(e)=-C({x_1})C(e).$$
% % But $\underline C\cap \underline X'=\{e,x_1\}$, and hence, again by orthogonality, $$X'(p)X'(x)=-C({x_1})C(e).$$
% % 
% % Finally, for the circuits with $X(p)\neq 0$ and $X({x_1})\neq 0$, since they are contravariant, $X(p)=-X({x_1})$. Observe that the rest of values of $X$ correspond to circuits of $\tilde \cP/\{p,x_1\}$. If all those circuits are halving, we are done.
% % 
% % By Lemma~\ref{lem:quotientsofShemersewing}, $\tilde \cP/\{p,x_1\}\simeq \cP/T_1[\cT/T_1]$. Since $\{x_1,y_1\}$ was a universal edge, $\cP/\{T_1\}$ is a neighborly matroid and $\cT/T_1$ is a universal flag. Then the result follows by induction. Observe for the base case, that all acyclic universal matroids of rank $1$ or $2$ are neighborly.
% % The second claim of the theorem is also a direct consequence of Lemma~\ref{lem:quotientsofShemersewing}.
% % This last proof by induction gives also directly claim~\eqref{it:newunifaces}. 
% \end{proof}
% 
% For matroids of odd rank, the flags of the previous theorem are the only ones that can yield a neighborly polytope.
%  
% \begin{proposition}\label{prop:uniqueflags}
% Let $\cP$ be a uniform neighborly oriented matroid of rank $d=2m+1$ with more than $d+1$ elements and with a flag $\cT$, and let $\tilde \cP=\cP[\cT]$, with $p$ sewn onto $\cP$ through~$\cT$. Then $\tilde \cP$ is neighborly if and only if $\cT$ contains a universal subflag.
% \end{proposition}
% \begin{proof}
% By Theorem~\ref{thm:extshemersewing}, this condition is sufficient.
% To find necessary conditions, we use that $\tilde \cP$ is neighborly if and only if every circuit of $\tilde \cP$ is halving.
% 
% By definition, $\tilde \cP=\cP[\cT]=\cP \cup p$ is a lexicographic extension of the form
% \(\tilde \cP= \cP\left[a_1^{+},\;a_2^{s_2},\dots,\;a_d^{s_d}\right]\). 
% Let $X\in\ci(\tilde\cP)$ be a circuit with $\{p,a_1\}\subset\underline X$.
% % $X(p)\neq 0$ and $X({a_1})\neq 0$. 
% Since $p$ and $a_1$ are contravariant, $X(p)=-X({a_1})$. Hence, if $X$ is balanced, so must be $X\setminus \{p,a_1\}$. Observe that %the remaining values of $X$ form 
% $X\setminus \{p,a_1\}$ is a circuit of $\tilde \cP/\{p,a_1\}$ and that all the circuits of $\tilde \cP/\{p,a_1\}$ arise this way. Hence $\tilde \cP/\{p,a_1\}$ must be neighborly.
% 
% By Proposition~\ref{prop:allquotientsofle}, \begin{equation*}\label{eq:Pquopa1}\tilde \cP/\{p,a_1\}\simeq \cP/\{a_1,a_2\}\left[a_3^{-s_2s_3},\;a_4^{-s_2s_4},\;,\dots,\;a_d^{-s_2s_d}\right].\end{equation*}
% Observe that $a_2$ and $a_3$ are $(s_2s_3)$-inseparable in $\tilde \cP/\{p,a_1\}$, which is a neighborly matroid of odd rank and corank at least~$2$. By Lemma~\ref{lem:balonlycovar}, $s_2s_3=-$.
% % 
% %  and Lemma~\ref{lem:circinseparable}, if $s_2s_3=+$ then there is a circuit $Y'$ of $\cP/\{p,a_1\}$ with $|Y^+|=|Y'^+|-1$. But then $Y$ and $Y'$ cannot be both halving, and thus $\cP/\{p,a_1\}$ can be neighborly only if $s_2s_3=-$.
% 
% % 
% % Let $Y$ be a circuit of $\tilde \cP/\{p,a_1\}$ with $Y(a_2)\neq 0$ and $Y(a_3)=0$. 
% % By Proposition~\ref{prop:allquotientsofle}, \begin{equation*}\label{eq:Pquopa1}\tilde \cP/\{p,a_1\}\simeq \cP/\{a_1,a_2\}\left[a_3^{-s_2s_3},\;a_4^{-s_2s_4},\;,\dots,\;a_d^{-s_2s_d}\right].\end{equation*}
% % Using this characterization and Lemma~\ref{lem:circinseparable}, if $s_2s_3=+$ then there is a circuit $Y'$ of $\cP/\{p,a_1\}$ with $|Y^+|=|Y'^+|-1$. But then $Y$ and $Y'$ cannot be both halving, and thus $\cP/\{p,a_1\}$ can be neighborly only if $s_2s_3=-$.
% 
% In particular, either $s_2=+$ and $s_3=-$, or $s_2=-$ and $s_3=+$. The first option implies that $T_1=\{a_1,a_2\}$, while the second option implies that $T_1=\{a_1\}$ and $T_2=\{a_1,a_2\}$. Moreover, if $\tilde \cP/\{p,a_1\}$ is neighborly, then $(\tilde \cP/\{p,a_1\})\setminus a_2\simeq\cP/\{a_1,a_2\}$ must be neighborly and hence $\{a_1,a_2\}$ must be a universal edge of $\cP$. 
% 
% Now the result follows by induction on $d$. For the base case just observe that neighborly matroids of rank $3$ are polygons, and the only 
% flags that yield a polygon with one extra vertex are of the form $\{x\}\subset \{x,y\}$ or just $\{x,y\}$, where $\{x,y\}$ is an edge of the polygon.
% %  Since any edge of a polygon is a universal edge, the only flag that does not adjust to our theorem is that containing only a $0$-face $\cT=\{T_1\}=\{\{x\}\}$. But if $p$ is sewn onto this $\cT$, then $x$ is not a vertex of the matroid anymore, and hence it cannot be neighborly.
% \end{proof}
% 
% 
% \begin{figure}[htpb]
% \begin{center}
% \includegraphics[width=.85\textwidth]{Figures/sewing.pdf}
% \end{center}
%  \caption[Sewing example]{Sewing onto $\{A,E\}$ (middle) and sewing onto $\{A\}\subset \{A,E\}$ (right). In the first case, $\{A,F\}$ and $\{E,F\}$ become universal faces, and $\{A,E\}$ is not a universal face any more. In the second case, $\{A,F\}$ and $\{A,E\}$ are universal faces, while $\{E,F\}$ is not.  }
%  \label{fig:sewing}
% \end{figure}
% 
% We can tell many universal faces (and flags) of the neighborly polytopes constructed using Theorem~\ref{thm:extshemersewing} thanks to Proposition~\ref{prop:extnewunifaces}, which is the analogue of point~\ref{it:newunifaces} of Theorem~\ref{thm:shemersewing}.
% %  for Theorem~\ref{thm:extshemersewing}.
% 
% We use the following notation. If $\cT'=\{T_j'\}_{j=1}^k$ is a flag of $\cP$ that contains a universal subflag $\cT=\{T_j\}_{j=1}^m$, where $T_j=\{x_i,y_i\}_{i=1}^{j}$, 
% we will say that $T_{i}$ is \defn{$x_i$-split} (resp. \defn{$y_i$-split}) if $T_{i-1}\cup\{x_i\}$ (resp. $T_{i-1}\cup\{y_i\}$) belongs to $\cT'$. 
% % observe that $\cT'$ is either like $\dots T_{i-1}\subset T_{i-1}\cup \{x_i\}\subset T_i\subset \dots$, like $\dots T_{i-1}\subset T_{i-1}\cup \{y_i\}\subset T_i\subset \dots$ or like 
% % $\dots T_{i-1}\subset T_i\subset \dots$. In the first two cases, 
% % we will say that $T_{i}$ is \defn{$x_i$-split} or \defn{$y_i$-split} respectively. 
% Moreover, we say that $T_i$ is \defn{even} if the number of non-split faces $T_j$ with $j\leq i$ is even, otherwise we say that $T_i$ is \defn{odd}.
% 
% \begin{proposition}\label{prop:extnewunifaces}
% Let $\cP$ be a uniform neighborly oriented matroid of rank $d$ with a flag $\cT'=\{T_j'\}_{j=1}^k$ that contains a universal subflag $\cT=\{T_j\}_{j=1}^m$, where $T_j=\{x_i,y_i\}_{i=1}^{j}$ and $m=\ffloor{d-1}{2}$. Let $\tilde \cP=\cP[\cT']$, with $p$ sewn onto $\cP$ through~$\cT'$. 
% Then the following are universal faces of $\tilde \cP$:
% \begin{enumerate}
%  \item\label{it:extnewuf1} $T_i$, where $1\leq i \leq m$, if $T_i$ is even.
%  \item $(T_{j}\setminus{x_i})\cup p$, where $1\leq i\leq j\leq m$, if
%       \begin{enumerate}[(i)]
% 	\item\label{it:extnewuf21} $T_i$ is not split and $T_j/T_i$ is even, or
% 	\item\label{it:extnewuf22} $T_i$ is $x_i$-split and $T_j/T_i$ is odd, or
% 	\item\label{it:extnewuf23} $T_i$ is $y_i$-split and $T_j/T_i$ is even.
%       \end{enumerate}
%  \item $(T_{j}\setminus{y_i})\cup p$, where $1\leq i\leq j\leq m$, if
%       \begin{enumerate}[(i)]
% 	\item\label{it:extnewuf31} $T_i$ is not split and $T_j/T_i$ is even, or
% 	\item\label{it:extnewuf32} $T_i$ is $x_i$-split and $T_j/T_i$ is even, or
% 	\item\label{it:extnewuf33} $T_i$ is $y_i$-split and $T_j/T_i$ is odd.
%       \end{enumerate}
% \end{enumerate}
% 
% \end{proposition}
% \begin{proof}
% Without loss of generality, we will assume that all split faces are $x_i$-split.
% The proof relies on applying, case by case, Proposition~\ref{prop:allquotientsofle} to reduce the contraction to a lexicographic extension that we know to be neighborly because of Theorem~\ref{thm:extshemersewing}.
% We also use the following observation about the signature of the extension $\cP[\cT']$: the sign of $x_i$ is $+$ if and only if $T_{i-1}$ is even. This follows from the fact that 
% \begin{equation*}
% \tilde \cP=
% \begin{cases}
% \cP[\dots,a^\alpha,x_i^{-\alpha},y_i^{\alpha},b^{-\alpha},\dots]& \text{ if $T_i$ is $x_i$-split,}
% \\
% \cP[\dots,a^\alpha,x_i^{-\alpha},y_i^{-\alpha},b^{\alpha},\dots]&\text{ if it is not split.}
% \end{cases}
% \end{equation*}
% In particular, if $T_i$ is even, $\tilde \cP/T_i =\cP/T_i[\cT'/T_i]$, and $T_i$ is a universal flag. This proves point~\ref{it:extnewuf1}.
% Moreover, independently of whether $T_i$ is even or odd, 
% %$\tilde \cP/(T_{i-1}\cup \{p\})\simeq \tilde \cP/(T_{i-1}\cup \{p,x_i\})$ 
% \begin{equation*}
% \tilde \cP/(T_{i-1}\cup \{p\})\simeq  
% \begin{cases}
%  \cP/(T_{i-1}\cup \{x_i\})[y_i^{+},x_{i+1}^{-},\dots]& \text{ if $T_i$ is split,}
% \\
%  \cP/(T_{i-1}\cup \{x_i\})[y_i^{-},x_{i+1}^{+},\dots]& \text{ if it is not.}
% \end{cases}
% \end{equation*}
% 
% Hence, $\tilde \cP/(T_{i-1}\cup \{x_i,p\})\simeq \cP/T_i[\cT'/T_i]$. If $T_i$ is not split $\tilde \cP/(T_{i-1}\cup \{y_i,p\})\simeq \cP/T_i[\cT'/T_i]$. Moreover, we know that $T_j/T_i$ is a universal face of $\cP/T_i[\cT'/T_i]$ when it is even. This proves points~\ref{it:extnewuf21}, \ref{it:extnewuf23}, \ref{it:extnewuf31} and \ref{it:extnewuf32}.
% 
% If $T_i$ is split, then $\tilde \cP/(T_{i-1}\cup \{y_i,p\})\simeq \cP/T_i[-\cT'/T_i]$, where $[-\cT'/T_i]$ means the extension $[\cT'/T_i]$ with the signs reversed. And using the previous observation, $\cP/T_i[-\cT'/T_i]/(T_j/T_i)\simeq \cP/T_j[\cT'/T_j]$ when $T_j/T_i$ is odd.
% Which proves the remaining points~\ref{it:extnewuf22} and \ref{it:extnewuf33}.
% \end{proof}
% 
% In particular, Proposition~\ref{prop:extnewunifaces} provides a simple way to tell universal flags of $\cP[\cT']$. If $T_1$ is not split then $\{x_1,p\}$ and $\{y_1,p\}$ are universal edges of $\cP[\cT']$; if it is $x_1$-split, then $\{x_1,p\}$ and $\{x_1,y_1\}$ are universal edges of $\cP[\cT']$; and if it is $y_1$-split, then $\{y_1,p\}$ and $\{x_1,y_1\}$ are universal edges of $\cP[\cT']$. Contracting any of these edges leaves a matroid isomorphic to $\cP/T_1[\cT'/T_1]$, and we can inductively build a universal flag of $\cP[\cT']$. The rank~$3$ example in Figure~\ref{fig:sewing} can give some intuition on why these universal edges appear.
% 
% \begin{example}
%  Let $\cM$ be a neighborly oriented matroid of rank~$5$ with a universal tower $\cT=\{a,b\}\subset\{a,b,c,d\}$. Consider the following lexicographic extensions 
% \begin{align*}
% p_1&=[a^+,b^+,c^-,d^-,e^+],\\p_2&=[a^+,b^-,c^+,d^+,e^-],\\p_3&=[a^+,b^+,c^-,d^+,e^-]\text{ and }\\p_4&=[a^+,b^-,c^+,d^-,e^+],
% \end{align*}
% where $e$ is any element of $\cM$. They give rise to the oriented matroids $\cM_1=\cM[p_1]$, $\cM_2=\cM[p_2]$, $\cM_3=\cM[p_3]$ and $\cM_4=\cM[p_4]$.
% 
% The following table shows for which $\cM_i$ is each of the following sets of vertices a universal face.
% 
% \centering
% \begin{tabular}{c|cccccccc}
% 	&$ab$&$p_ib$&$ap_i$&$abcd$&$p_ibcd$&$ap_icd$&$abp_id$&$abcp_i$\\\hline
% $\cM_1$&\cross&\tick&\tick&\tick&\cross&\cross&\tick&\tick\\
% $\cM_2$&\tick&\cross&\tick&\cross&\tick&\cross&\tick&\tick\\
% $\cM_3$&\cross&\tick&\tick&\cross&\tick&\tick&\cross&\tick\\
% $\cM_4$&\tick&\cross&\tick&\tick&\cross&\tick&\cross&\tick 
% \end{tabular}
%  
% \end{example}
% 
% 
% % \begin{remark}
% %  The sewing construction is not the only lexicographic extension that extends a neighborly matroid to another neighborly matroid.
% %  For example, in \cite{LeeMenzel2010}, Lee and Menzel prove the following result: let $\cP$ be the matroid of a cyclic polytope $\cyc{n}{d}$ with elements $s_1,\dots,s_n$ labeled in cyclic order, and let~$\cT$ be the flag $\cT=\{s_n\}\subset\{s_{n-1},s_n\}\subset \dots \subset\{s_{n-d+1},\dots,s_n\}$. Then $\cP[\cT]$ is the matroid of the cyclic polytope $\cyc{n+1}{d}$.
% % \end{remark}
% \begin{remark}
%  Theorem~\ref{thm:extshemersewing} not only generalizes the Sewing Theorem. It also includes Barnette's facet-splitting technique~\cite[Theorem 3]{Barnette1981}.
% \end{remark}
% 
% 
% Just like we did to construct the family \defn{$\cS$}, we can combine Example~\ref{ex:universalflagsofcyclic}, Theorem~\ref{thm:extshemersewing}
% and Proposition~\ref{prop:extnewunifaces} to obtain a large family of neighborly polytopes that contains $\cS$. We call this family $\cE$.
% In fact, since \cite[Theorem 5.1]{LeeMenzel2010} implies that cyclic polytopes belong to $\cE$, it is enough to start sewing on a simplex.
% 
% 
% Moreover, since every subpolytope of a neighborly polytope is a neighborly polytope, any polytope obtained from a polytope in $\cE$ and then omitting some vertices is also a neighborly polytope. The polytopes that can be obtained this way via sewing and omitting form a family that we denote \emph{$\cO$}. 
% 
% % 
% % \begin{proposition}
% %  $\cE\subset \cO$.
% % \end{proposition}
% % \begin{proof}
% % \ojo{TO DO. To finish, not sure if it is true.}
% % 
% %  Let $\tilde \cP$ be in $\cE$. That is, there is $\cP\in \cE$ such that $\tilde \cP=\cP[\cT']$ for a flag $\cT'$ with a universal subflag $\cT=\{T_j\}_{j=1}^m$, where $T_j=\{x_i,y_i\}_{i=1}^{j}$. Assume that all the split faces of $\cT'$ are $x_i$-split, and call $p$ the sewn vertex.
% %  
% %  Let $x_1'$ be sewn onto $\cP$ through $\cT$. Let $\tilde T_i=T_{i-1}\cup x_1' \cup y_i$ if $T_i$ is not split and $\tilde T_i=T_{i-1}\cup x_1' \cup x_i$ if $T_i$ is split. By Proposition~\ref{prop:extnewunifaces}, $\tilde\cT$ is a universal flag of $\cP[\cT]$.
% %  Let $p'$ be sewon onto $\cP[\cT]$ onto $\tilde\cT$.
% %   
% %  We claim that $\cP[\cT']\simeq\cP[\cT][\tilde \cT]\setminus x_1$ where $x_1\mapsto x_1'$ and $p\mapsto p'$.
% % 
% %  The first observation is that $\cP\simeq \cP[\cT]\setminus x_1$ where $x_1\mapsto x_1'$, just because $x_1$ and $x_1'$ are contravariant in $\cP[\cT]$. Hence, it is enough to see that the signature of $p$ in $\cP$, $\sigma$, coincides with the signature of $p'$ in $\cP[\cT]\setminus x_1$, $\sigma'$.
% %   
% %  Let $C\in \co(\cP)$ with $C(x_1)\neq 0$, and let $C'\in \co(\cP[\cT])$ be the extension of $C$ (hence $C'(x_1)\neq 0$ and $C'(x_1')\neq 0$). Then $\sigma(C)=C(x_1)$ and $\sigma'(C')=C'(x_1')=C(x_1)$ because $x_1'$ and $x_1$ are contravariant in $\cP[\cT]$.
% % 
% %  Let $C\in \co(\cP)$ with $C(x_1)=0$ and $C(y_1)\neq0$, and let $C'\in \co(\cP[\cT])$ be the cocircuit with $\underline C'=\underline C \cup x_1$. Since $C'(x_1)= 0$, it is a cocircuit of $\cP[\cT]/x_1'$.
% % 
% %  If $T_1$ is not split, then $\sigma(C)=C(y_1)$. Moreover, $\tilde T_1=\{x_1',y_1\}$ and hence $\sigma'(C')=C'(y_1)=C(y_1)$.
% % 
% %  If $T_1$ is split, then $\sigma(C)=-C(y_1)$. Moreover, since $\cP[\cT]/x_1'\simeq \cP/x_1[y_1^-,\dots]$ and since $\tilde T_1=\{x_1',x_1\}$, then $\sigma'(C')=C'(x_1)=-C(y_1)$.
% % 
% %  Finally, let $C\in \co(\cP)$ with $C(x_1)=0$ and $C(y_1)=0$, and $C'\in \co(\cP[\cT])$ with $\underline C'=\underline C \cup x_1$. 
% %  
% %  If $T_1$ is not split, the signature $\sigma(C)$ coincides with the signature of the extension $\cP[\cT]/T_1\simeq\cP/T_1[-\cT'/T_1]$. The singature $\sigma'(C')$ coincides with the signature of the extension 
% % $\cP[\cT][\tilde \cT]/\{x_1',y_1\}\setminus x_1\simeq\cP/T_1[-\cT/T_1][\tilde \cT/T_1]\setminus x_1$
% % 
% % 
% % \end{proof}
% 

% \thispagestyle{empty}
% \chapter{The Gale sewing construction}\label{ch:thethm}
% 
% We present here a different construction, also based on lexicographic extensions, that allows us to construct neighborly matroids. This construction works in the dual, that is, it extends balanced matroids to new balanced matroids.
% %  With the tools that we have already presented, it is extremely simple to understand and prove.
% 
% % \begin{lemma}
% % Let $\cM$ be an oriented matroid of rank $r$, let $p$ be a lexicographic extension on $[a_1^{s_1},a_2^{s_2},\dots,a_r^{s_r}]$, and let $q$ be a lexicographic extension of $\cM\cup p$ on $[p^-,a_1^{-},\dots,a_{r-1}^{-}]$. Finally, let $\tilde \cM=\cM\cup p\cup q$. Then $\disc(\tilde \cM)=\disc(\cM)$. 
% % \end{lemma}
% % \begin{proof}
% % We prove that $\disc(\tilde \cM)=\disc(\cM)$ by checking that all the cocircuits $\tilde C$ of $\tilde \cM$ have the same discrepancy as some cocircuit of $\cM$.
% % 
% % If $\tilde C(p)\neq 0$ and $\tilde C(q)\neq 0$ then, by definition of the lexicographic extension, there is a cocircuit $C$ of $\cM$ such that $\restriction{\tilde C}{\cM}=C$ and $C(p)=-C(q)$. Hence $|\tilde C^+|=|C^+|+1$ and $|\tilde C^-|=|C^-|-1$.
% % 
% % The cocircuits $\tilde C$ with $\tilde C(p)=0$ correspond to cocircuits of $\tilde \cM/p$, and those with $\tilde C(q)=0$ correspond to cocircuits of $\tilde \cM/q$. 
% % % And are halving since $\tilde \cM/p$ and $\tilde \cM/q$ are balanced. 
% % The result follows by induction on $r$ (it is trivial for $r=1$), since Proposition~\ref{prop:allquotientsofle} tells us that 
% % \begin{displaymath}\tilde \cM/p\simeq \tilde \cM/q\simeq\cM/a_1[a_2^{-s_1s_2},\dots,a_r^{-s_1s_2}][p^-,a_2^-,\dots,a_{r-1}^-].\end{displaymath} 
% % \end{proof}
% 
% % \begin{proof}
% % Let $\tilde C$ be a cocircuit of $\tilde \cM$ that contains nor $p$ neither $q$ in $\tilde C^0$. Then, there is a cocircuit $C$ of $\cM$ such that $\restriction{\tilde C}{\cM}=C$
% % , and $C(p)=-C(q)$, by definition of the lexicographic extension. Hence $|\tilde C^+|=|C^+|+1$ and $|\tilde C^-|=|C^-|-1$.
% % 
% % The cocircuits with $p\in C^0$ correspond to those of $\tilde \cM/p$, and those with $q\in C^0$ correspond to those of $\tilde \cM/q$.
% % 
% % Finally, Proposition~\ref{prop:allquotientsofle} tells us that $\tilde \cM/p\simeq \tilde \cM/q\simeq\cM/a_1[a_2^{-s_1s_2},\dots,a_r^{-s_1s_2}][p^-,a_2^-,\dots,a_{r-1}^-]$, and the result follows by induction on $r$ (it is trivial for $r=1$).
% % \end{proof}
% % 
% %  And as a direct corollary:
% 
% \begin{proposition}
% Let $\cM$ be a uniform oriented matroid of rank $r$, let $p$ be a lexicographic extension on $[a_1^{s_1},a_2^{s_2},\dots,a_r^{s_r}]$, and let $q$ be a lexicographic extension of $\cM\cup p$ on $[p^-,a_1^{-},\dots,a_{r-1}^{-}]$. If $\tilde \cM=\cM\cup p\cup q$, then $\disc(\tilde \cM)=\disc(\cM)$. 
% \end{proposition}
% \begin{proof}
% We prove that $\disc(\tilde \cM)=\disc(\cM)$ by checking that every cocircuit $\tilde C$ of $\tilde \cM$ has the same discrepancy as some cocircuit of $\cM$.
% 
% If $\tilde C(p)\neq 0$ and $\tilde C(q)\neq 0$ then, by the definition of lexicographic extension, there is a cocircuit $C$ of~$\cM$ such that $\restriction{\tilde C}{\cM}=C$ and $\tilde C(p)=-\tilde C(q)$. Hence $|\tilde C^+|=|C^+|+1$ and $|\tilde C^-|=|C^-|+1$.
% 
% The cocircuits $\tilde C$ with $\tilde C(p)=0$ correspond to cocircuits of $\tilde \cM/p$, and those with $\tilde C(q)=0$ correspond to cocircuits of $\tilde \cM/q$. 
% % Both are halving since $\tilde \cM/p$ and $\tilde \cM/q$ are balanced; indeed, 
% Proposition~\ref{prop:allquotientsofle} tells us that 
% \begin{displaymath}\tilde \cM/p\simeq \tilde \cM/q\simeq\cM/a_1[a_2^{-s_1s_2},\dots,a_r^{-s_1s_2}][p^-,a_2^-,\dots,a_{r-1}^-],\end{displaymath} and the result follows by induction on $r$ (it is trivial for $r=1$).
% \end{proof}
% 
% In a vector configuration $V$, the proof that $V[p][q]$ has the same discrepancy as $V$ is very easy to understand. For every hyperplane $h$ spanned by $V$, if $p\in h^+$ then $q\in h^-$, and hence $q$ balances the discrepancy created by $p$. For a hyperplane $h$ that goes through $p$ but neither $a_1$ nor $q$, the fact that $p$ and $a_1$ are inseparable implies that except for $a_1$, $h$ looks like a hyperplane spanned by $V$ going through $a_1$. Hence $q$ must balance the discrepancy created by $a_1$. For hyperplanes that go through $p$ and $a_1$ but not $a_2$ nor $q$, $q$ balances the discrepancy created by $a_2$. And so on.
% 
% And as a direct corollary:
% \begin{theorem}\label{thm:thethm}
%  Let $\cM$ be a uniform balanced oriented matroid of rank $r$, let $p$ be a lexicographic extension on $[a_1^{s_1},a_2^{s_2},\dots,a_r^{s_r}]$, and let $q$ be a lexicographic extension of $\cM\cup p$ on $[p^-,a_1^{-},\dots,a_{r-1}^{-}]$. Then $\cM\cup p\cup q$ is balanced. 
% \end{theorem}
% 
% This provides the following construction to construct balanced matroids (and hence, by duality, to construct neighborly matroids). 
% Let $\cM_0=\stc{r}$ be the oriented matroid associated to the totally cyclic vector configuration of rank $r$ of minimal cardinality, which is balanced. And let
% \begin{align*}
% x_k&=[e_{k1}^{s_{k1}},\dots,e_{kr}^{s_{kr}}],& y_k&=[x_k^-,e_{k1}^{-},\dots,e_{k(r-1)}^{-}],%\\
% &\cM_k&=\cM_{k-1}[x_k][y_k], 
% \end{align*}
% where each $e_{ij}$ is a different element of $\cM_{i-1}$. Then $\cM_k$ is balanced, and $\cM_k^*$ neighborly. Since $\cM_0$ is realizable, $\cM_k^*$ is too, and hence $\cM_k^*$ represents a neighborly polytope.
% 
% We call the double extension of Theorem~\ref{thm:thethm} \emph{Gale sewing}, and we denote by \emph{$\cG$} the family of polytopes whose dual is constructed by repeatedly Gale sewing from some $\cD_r$.
% 
% % \begin{remark}
% %  Gale sewing can be applied onto any balanced matroid. In particular, it can be used to construct infinitely many non-realizable neighborly oriented matroids, just by starting from a non-realizable neighborly oriented matroid.
% % \end{remark}
% % \begin{remark}
% % On a non-necessarily balanced matroid, Gale sewing preserves discrepancy. 
% % \end{remark}
% 
% \begin{corollary}\label{cor:primalGaleSewing}
%  Let $\cP$ be a neighborly matroid of rank $d$ and $n$ elements, then there exists a neighborly matroid $\tilde \cP$ of rank $d+2$ with $n+2$ elements with two distinguished elements $x$ and $y$ such that $\tilde\cP/\{x,y\}=\cP$.
% \end{corollary}
% 
% 
% Cyclic polytopes are a first example of polytopes in $\cG$. 
% \begin{proposition}\label{prop:cyclicaregalesewn}
% % \begin{proposition}
%  Let $\cM$ be an oriented matroid dual to a cyclic polytope $\cyc{d}{n}$, with elements $s_1,s_2,\dots, s_n$ labeled according to the cyclic order. Then $\cM\cup\{x\}=\cM[s_{n}^-,s_{n-1}^-,\dots,s_{d}^-]$ is an oriented matroid dual to $\cyc{d+1}{n+1}$, with $x=s_{n+1}$.
% % If $x$ is Gale sewn onto $S$ through $[s_{n}^-,s_{n-1}^-,\dots,s_{d}^-]$, then $\cM\cup\{x\}$ is an oriented matroid dual to $\cyc{d+1}{n+1}$, with $x=s_{n+1}$.
% % \end{proposition}
% \end{proposition}
% \begin{proof}
%  The circuits of the cyclic polytope are as follows: the circuits $X$ and $Y$ supported by the $r+1$ points $e_1<e_2<\dots<e_{r+1}$ are $X(e_i)=(-1)^i$ and $Y(e_i)=(-1)^{i+1}$ \cite[Section 9.4]{OrientedMatroids1993}.
%  
%  If $C$ is a cocircuit of $\cM[x]$ (hence a circuit of its dual), the signature of the lexicographic extension implies that $C(x)$ is opposite to the sign of the largest non-zero element. And thus $\cM\cup x$ is dual to $\cyc{d+1}{n+1}$. 
% \end{proof}
% 
% When Gale sewing, one can interchange the role of $a_1$, $p$ and $q$ as follows. 
% 
% \begin{lemma}\label{lem:galesewingorder}
% Let $\cM$ be a uniform oriented matroid on a ground set $E$, and consider the lexicographic extensions
% \begin{align*}
%  p&=[a_1^{s_1},\dots,a_r^{s_r}],& q&=[p^-,a_1^{-},\dots,a_{r-1}^{-}];\\
%  p'&=[a_1^{-s_1},\dots,a_r^{-s_r}],& q'&=[p'^-,a_1^{-},\dots,a_{r-1}^{-}];\\
%  p''&=[a_1^{+},a_2^{-s_1s_2},\dots,a_r^{-s_1s_r}],& q''&=[p''^-,a_1^{-},\dots,a_{r-1}^{-}].
% \end{align*}
% Then,
%  \begin{align}
% \cM[p][q]&\stackrel{\varphi}{\simeq}\cM[p'][q'],\text{ and }\label{eq:changepq}\\  \cM[p][q]&\stackrel{\psi}{\simeq}\cM[p''][q''],  \label{eq:changepa1} 
%  \end{align}
% where $\varphi(p)=q'$, $\varphi(q)=p'$ and $\varphi(e)=e$ for $e\in E$. If $s_1=+$, then $\psi(p)=a_1$, $\psi(q)=q''$, $\psi(a_1)=p''$ and $\psi(e)=e$ for $e\in E\setminus\{a_1\}$, and if $s_1=-$, then $\psi(p)=q''$, $\psi(q)=a_1$, $\psi(a_1)=p''$ and $\psi(e)=e$ for $e\in E\setminus\{a_1\}$
% \end{lemma}
% \begin{proof}
% We start proving $\cM[p][q]\stackrel{\varphi}{\simeq}\cM[p'][q']$. That is, for every cocircuit $C\in\co(\cM[p][q])$ we want to find a cocircuit $C'\in\co(\cM[p'][q'])$ with $C'(\varphi(a))=C(a)$ for all $a\in E\cup\{p,q\}$, that is $C'(p')=C(q)$, $C'(q')=C(p)$ and $C'(e)=C(e)$ for $e\in E$. Let $D$ be the restiction of $C$ to $E$.
% 
% If $C(q)\neq 0$ and $C(p)\neq 0$, let $i$ be minimal with $D(a_i)\neq 0$. By construction, $C(p)=s_iD(a_i)$ and $C(q)=-C(p)=-s_iD(a_i)$. By the definition of $\cM[p'][q']$, there is a cocircuit $C'$ that expands $D$, with $C'(p')=-s_iD(a_i)$ and $C'(q')=-C(p')=s_iD(a_i)$.
% 
% To deal with the case when $C(q)= 0$ or $C(p)= 0$, by induction it is direct to see that $\cM[p][q]/p{\simeq}\cM[p'][q']/q'$ and that $\cM[p][q]/q{\simeq}\cM[p'][q']/p'$.
% 
% Now, to see that $\cM[p][q]\stackrel{\psi}{\simeq}\cM[p''][q'']$ we can assume that $s_1=+$, otherwise we use eq.~\eqref{eq:changepq} to change the order of $p$ and $q$. In this case we will prove that \(\cM[p]\simeq\cM[p'']\). This suffices to prove eq.~\eqref{eq:changepa1} since $[p^-,a_1^{-},\dots,a_{r-1}^{-}]$ and $[a_1^-,p^-,\dots,a_{r-1}^{-}]$ give the same signature when $p$ and $a_1$ are contravariant.
% 
% For every cocircuit $C\in\co(\cM[p])$ we want to find now a cocircuit $C''\in\co(\cM[p''])$ with $C''(p'')=C(a_1)$, $C''(a_1)=C(p'')$ and $C''(e)=C(e)$ for $e\in E\setminus\{a_1\}$. Again, let $D$ be the restriction of $C$ to $E$.
% 
% If $C(p)\neq 0$ and $C(a_1)\neq 0$, then $C(p)=C(a_1)=D(a_1)$. And $D$ can also be expanded to a cocircuit $C''$ of $\cM[p'']$ with $C''(p'')=C''(a_1)=D(a_1)$. For circuits with $C(p)\neq 0$ and $C(a_1)=0$, then $\cM[p]/a_1=\cM[a_2^{s_2},\dots,a_r^{s_r}]{\simeq}\cM[p'']/p''$ by Proposition~\ref{prop:allquotientsofle}. Finally, if $C(p)= 0$ and $C(a_1)\neq 0$, then, again by Proposition~\ref{prop:allquotientsofle}, $\cM[p]/p{\simeq}\cM[a_2^{-s_2},\dots,a_r^{-s_r}]=\cM[p'']/a_1$.
% \end{proof}
% 
% 
% Using Proposition~\ref{prop:allquotientsofle}, we obtain the following result that explains the contractions of Gale sewing extensions:
% 
% \begin{lemma}\label{lem:quotientsofGalesewnareGalesewn}
% Let $\cM$ be a uniform oriented matroid of rank $r$, and consider the lexicographic extensions
% \begin{align*}
% p&=[a_1^{s_1},a_2^{s_2},\dots,a_r^{s_r}],&q&=[p^-,a_1^{-},\dots,a_{r-1}^{-}];\\
% p'&=[a_2^{-s_1s_2},\dots,a_r^{-s_1s_r}],& q'&=[p'^{-},\dots,a_{r-1}^{-}].
% \end{align*}
% 
% Then \begin{math}\left(\cM[p][q]\right)/q\simeq\left(\cM/a_1\right)[p'][q'].\end{math}
% \end{lemma}
% \begin{proof}
% Repeatedly applying Proposition~\ref{prop:allquotientsofle},
% \begin{align*}
% \left(\cM[p][q]\right)/q&= \big(\cM\underbrace{[a_1^{s_1},a_2^{s_2},\dots,a_r^{s_r}]}_{p}\underbrace{[p^-,a_1^{-},\dots,a_{r-1}^{-}]}_{q}\big)/q\\
% &\stackrel{\varphi}{\simeq} \big(\cM\underbrace{[a_1^{s_1},a_2^{s_2},\dots,a_r^{s_r}]}_{p}/p\big)\underbrace{[a_1^{-},\dots,a_{r-1}^{-}]}_{\varphi(p)=q'}\\
% &\stackrel{\psi}{\simeq} \big(\cM/a_1\big)\underbrace{[a_2^{-s_1s_2},\dots,a_r^{-s_1s_r}]}_{\psi(a_1)=p'}\underbrace{[\psi(a_1)^{-},\dots,a_{r-1}^{-}]}_{q'}.
% \end{align*}
% \end{proof}
% 
% 
% In fact, from this result and Proposition~\ref{prop:allquotientsofle}, it is easy to derive that subpolytopes of Gale sewn polytopes are also Gale sewn:
% 
% \begin{proposition}\label{prop:allquotientsofGalesewnareGalesewn}
%  Let $\cP$ be a neighborly polytope in $\cG$, and let $e$ be an element of $\cP$. Then $\cP\setminus e$ is also in $\cG$.
% \end{proposition}
% \begin{proof}
%  The proof is by induction on the rank of $\cP$. When $\cP$ has rank $0$ then $\cP^*=\cD_r$ and $(\cP\setminus e)^*=\cD_r/e=\cD_{r-1}$.
% 
%   Otherwise, let $\cM=\cP^*$. That $\cP$ belongs to $\cG$ means that there is a matroid $\cN$ whose dual $\cN^*$ corresponds to a polytope $\cQ$ in $\cG$, such that $\cM=\cN[p][q]$ where $p=[a_1^{s_1},a_2^{s_2},\dots,a_r^{s_r}]$ and $q=[p^-,a_1^{-},\dots,a_{r-1}^{-}]$. We will show that for every element $e$ of $\cP$, there is some element $e'$ of $\cN$ such that $(\cP\setminus e)^*\simeq (\cN/ e')[p'][q'] =(\cQ\setminus e')^*[p'][q']$. Since $\rank \cQ=\rank \cP -2$, by the induction hypothesis $(\cQ\setminus e')\in \cG$ and the result follows. 
% 
%  If $e=q$, then by Lemma~\ref{lem:quotientsofGalesewnareGalesewn}, $(\cP\setminus e)^*=\left(\cN[p][q]\right)/q\simeq\left(\cN/a_1\right)[p'][q']$. The case $e=p$ is analogous because of Lemma~\ref{lem:galesewingorder}.
% %  $\cP\setminus e$ is in $\cG$ because of Lemma~\ref{lem:galesewingorder} and Lemma~\ref{lem:quotientsofGalesewnareGalesewn}.
%  If $e=a_i$, then $\left(\cP\setminus e\right)^*\simeq\left(\cN/a_i\right)[p'][q']$, 
% where $p'$ and $q'$ have the same signature as $p$ and $q$ but omitting the element $a_i$.
% %  $p=[a_1^{s_1},a_2^{s_2},\dots,a_{i-1}^{s_{i-1}},a_{i+1}^{s_{i+1}},\dots, a_r^{s_r}]$, $q=[p^-,a_1^{-},\dots,a_{i-1}^{-},a_{i+1}^{-},\dots,a_{r-1}^{-}]$.
%  For the remaining elements $e$, $\left(\cP\setminus e\right)^*\simeq\left(\cN/e\right)[p][q]$.
% \end{proof}
% 
% 
% 
% % 
% % \begin{lemma}\label{lem:galesewingorder}
% % Let $\cM$ be an oriented matroid, and consider the lexicographic extensions
% % \begin{align*}
% %  p&=[a_1^{s_1},\dots,a_r^{s_r}],& q&=[p^-,a_1^{-},\dots,a_{r-1}^{-}];\\
% %  q'&=[a_1^{-s_1},\dots,a_r^{-s_r}],& p'&=[q'^-,a_1^{-},\dots,a_{r-1}^{-}].
% % \end{align*}
% % Then,
% %  \begin{math}\cM[p][q]\simeq\cM[q'][p']\end{math}
% % with the natural isomorphism.
% % \end{lemma}
% % \begin{proof}
% % We see first that the signature of $q'$ in $\cM$ is the same as the signature of $q$ in $\cM[p]\setminus p$. 
% % Let $C\in\co(\cM)$ be a cocircuit of $\cM$, and let $a_i$ be minimal with $C({a_i})\neq 0$. The signature of $q'$ is $\sigma'(C)=-s_iC(a_i)$. The signature of $p$ is $\sigma(C)=s_iC(a_i)$ and hence the signature of $q$ in the cocircuit $C'=(C,\sigma(C))$ of $\cM[p]$ is $-C'(p)=-s_iC(a_i)$, as we wanted to see. Analogously, the signature of $p$ in $\cM$ is the same as the signature of $p'$ in $\cM[q']\setminus q'$.
% % 
% % Hence, we just need to study the signatures of $q$ and $q'$ in the cocircuits of $\cM[p][q]$ and $\cM[q'][p']$ that take value $0$ in $p$ and $p'$. However, using Proposition~\ref{prop:allquotientsofle} it is direct to see by induction that $\cM[q'][p']/p'\simeq \cM[p][q]/p$.
% % \end{proof}
% % 
% % \begin{lemma}\label{lem:galesewingorder2}
% % Let $\cM$ be an oriented matroid, and consider the lexicographic extensions
% % \begin{align*}
% %  p&=[a_1^{+},a_2^{s_2}\dots,a_r^{s_r}],& q&=[p^-,a_1^{-},\dots,a_{r-1}^{-}];\\
% %  p'&=[a_1^{+},a_2^{-s_2},\dots,a_r^{-s_r}],& q'&=[p'^-,a_1^{-},\dots,a_{r-1}^{-}].
% % \end{align*}
% % Then,
% %  \begin{math}\cM[p][q]\simeq\cM[p'][q']\end{math}
% % with the isomorphism that maps $a_1\mapsto p'$, $p\mapsto a_1$ and $q\mapsto q'$.
% % \end{lemma}
% % \begin{proof}
% % In fact \(\cM[p]\simeq\cM[p']\). First of all, $\cM[p']\setminus a_1 \simeq \cM=\cM[p]\setminus p$, just because $a_1$ and $p'$ are contravariant. Hence, we just need to see that the signature of $p$ in $\cM$ is tha same as the signature of $a_1$ in $\cM[p']$. The elements $p$ and $a_1$ are contravariant in $\cM[p]$ just like $a_1$ and $p'$ are contravariant in $\cM[p']$. For cocircuits $C\in\co(\cM[p])$ with $C(a_1)= 0$, observe that the signature of $p$ is that of the lexicographic extension $[a_2^{s_2},\dots,a_r^{s_r}]$, which coincides with the signature of $a_1$ for cocircuits $C\in\co(\cM[p'])$ with $C(p)= 0$ because of Proposition~\ref{prop:allquotientsofle}.
% % 
% % To finish the proof we just need to observe that since $p$ and $a_1$ are contravariant, $[p^-,a_1^{-},\dots,a_{r-1}^{-}]$ and $[a_1^-,p^-,\dots,a_{r-1}^{-}]$ give the same signature.
% % \end{proof}
% 
% 
% \subsection{Combinatorial description of the polytopes in $\cG$}
% 
% Let $P$ be a polytope that defines an acyclic oriented matroid $\cP$, and let $\cM=\cP^*$ be its dual matroid. The essence of Gale sewing is to construct a new polytope $\tilde P$ whose matroid $\tilde \cP$ is dual to $\tilde\cM=\cM[p]$, a lexicographic extension of $\cM$ on $p=[a_1^{s_1},a_2^{s_2},\dots,a_k^{s_k}]$. In this section we will see that the combinatorics of $\tilde P$ are described by \defn{lexicographic triangulations} of $P$.
% 
% \begin{remark}
%  The resemblance with the description of the vertex figures of the neighborly cubical polytopes in~\cite{SanyalZiegler2010} is not a coincidence. Indeed, the duals of those vertex figures are lexicographic extensions of the dual of a fixed neighborly polytope.
% \end{remark}
% 
% Let $v_1,\dots,v_n$ be the vertices of $P\subset \RR^d$, and assume (reordering the $v_i$'s if necessary) that $a_i$ is the dual element corresponding to $v_i$. Let $V$ be the $n\times dn$ matrix whose rows list the coordinates of the $v_i$'s:
% 
% $$
%        V = 
%       \left[
%       \begin{array}{ccccc}
%             \multicolumn{5}{c}{\;\hrulefill\;v_1\;\hrulefill\;}\\
%             \multicolumn{5}{c}{\;\hrulefill\;v_2\;\hrulefill\;}\\
%             \quad&\quad&\vdots&\quad&\quad     \\
%             \multicolumn{5}{c}{\;\hrulefill\;v_{n}\;\hrulefill\;}   \\
%         \end{array}
% 	\right].	
% $$
% 
% 
% % If $\tilde \cM=\cM[a_1^{s_1},a_2^{s_2},\dots,a_k^{s_k}]$, then the $(n+1)\times(d+1)$ matrix that encodes the vertices of $\tilde P$ is the following matrix $\tilde V$ for some $\delta$ small enough.
% Then the following $(n+1)\times(d+1)$ matrix $\tilde V$ encodes the vertices of $\tilde P$, for some small enough $\delta$.
% 
% $$
%       \tilde V = 
%       \left[
%       \begin{array}{ccccc|c}
%             \multicolumn{5}{c|}{\;\hrulefill\;v_1\;\hrulefill\;} &-s_1\\
%             \multicolumn{5}{c|}{\;\hrulefill\;v_2\;\hrulefill\;} &-s_2 \delta \\
%             \multicolumn{5}{c|}{\;\hrulefill\;v_3\;\hrulefill\;} &-s_3\delta^2 \\
%             \quad&\quad&\vdots&\quad&\quad     &\vdots\\
%             \multicolumn{5}{c|}{\;\hrulefill\;v_k\;\hrulefill\;} &-s_k\delta^{k-1} \\
%             \multicolumn{5}{c|}{\;\hrulefill\;v_{k+1}\;\hrulefill\;} &0\\
%             \quad&\quad&\vdots&\quad&\quad     &\vdots\\
%             \multicolumn{5}{c|}{\;\hrulefill\;v_{n}\;\hrulefill\;}   &0\\%\cline{1-5}	
% 	    \multicolumn{5}{c|}{\;\hrulefill\;\veczero\;\hrulefill\;}   &1
%         \end{array}
% 	\right].
% $$
% 
% The vertex figure of $p$ in $\tilde P$ is combinatorially equivalent to $P$, hence the faces of $\tilde P$ that contain $p$ are isomorphic to pyramids over faces of $P$. On the other hand, the faces of $\tilde P$ that do not contain $p$ correspond to faces of a regular subdivision of $P$: a \emph{lexicographic subdivision} of $P$ on $[v_1^{-s_1},v_2^{-s_2},\dots,v_k^{-s_k}]$. %$[v_r^{-s_r},\dots,v_2^{-s_2},v_1^{-s_1}]$.
% When $k=r$, then this subdivision is a triangulation.
% 
% \begin{figure}[htpb]
% \begin{center}
% \includegraphics[width=\textwidth]{Figures/lifting.pdf}
% \end{center}
%  \caption[Lifting triangulation]{The lifting of a pentagon $P$ to $\tilde P$ when $p=[a_1^-,a_4^+]$. Its upper envelope are pyramids over facets of $P$, while the lower envelope is the lexicographic triangulation of $P$ on $[a_1^+,a_4^-]$. }
%  \label{fig:lifting}
% \end{figure}
% 
% Our formulation of the definition of lexicographic subdivision is based on~\cite{DeLoeraRambauSantosBOOK}. However we use a different ordering, the same as in~\cite{Santos2002}, that mirrors the definition of lexicographic extension. See also~\cite{Lee1991}.
% % The following exposition is based on~\cite{DeLoeraRambauSantosBOOK}\footnote{The exposition is based on~\cite{DeLoeraRambauSantosBOOK}, however the definition that we use here uses a different ordering, the same as in~\cite{Santos2002}, that mirrors the definition of lexicographic extension.}, and gives a recursive definition in terms of a sequence of operations of pushing and pulling.
% 
% \begin{definition}%[formulation from~\cite{DeLoeraRambauSantosBOOK}]
% Let $P$ be a $d$-polytope with $n$ vertices $v_1,\dots,v_n$. The \defn{lexicographic subdivision} of $P$ on $[v_1^{s_1},v_2^{s_2},\dots,v_k^{s_k}]$, where $s_i=\pm 1$, is defined recursively as follows.
% \begin{itemize}
%  \item If $s_1=+1$ (pushing), then the lexicographic subdivision of $P$ is the union of the lexicographic subdivision of $P\setminus v_1$ on $[v_2^{s_2},\dots,v_k^{s_k}]$, and the simplices joining $v_1$ to the (lexicographically subdivided) faces of $P\setminus v_1$ visible from it.
%  \item If $s_1=-1$ (pulling), then the lexicographic subdivision of $P$ is the unique subdivision in which every maximal cell contains $v_1$ and which, restricted to each proper face $F$ of $P$, coincides with the lexicographic subdivision of that face.
% \end{itemize}
% \end{definition}
% 
% % \begin{remark}
% %  It is not a coincidence the resemblance with the description of the vertex figures of the neighborly cubical polytopes in~\cite{SanyalZiegler2010}. Indeed, the duals of those vertex figures are lexicographic extensions of the dual of a fixed neighborly polytope.
% % \end{remark}
% 
% 
% % \subsection{Combinatorial description of the polytopes in $\cG$}
% % 
% % Let $P$ be a polytope that defines an acyclic matroid $\cP$, and let $\cM=\Gale{\cM}$ be its dual matroid, the objective of this section is to understand $\tilde\cP$, the dual to $\tilde\cM=\cM[p]$, where $p$ is a lexicographic extension on $[a_1^{s_1},a_2^{s_2},\dots,a_r^{s_r}]$. The combinatorics of the face lattice of $\tilde \cP$ are described by the combinatorics of the \emph{lexicographic triangulations} of $P$.
% % 
% % Let $v_1,\dots,v_n$ be the vertices of $P\subset \RR^d$, and assume (reordering the $v_i$'s if necessary) that $a_i$ is the dual element corresponding to $v_i$. Let $V$ be the $n\times dn$ matrix that encodes the coordinates of the $v_i$'s as rows:
% % 
% % $$
% %        V = 
% %       \left[
% %       \begin{array}{ccccc}
% %             \multicolumn{5}{c}{\;\hrulefill\;v_1\;\hrulefill\;}\\
% %             \multicolumn{5}{c}{\;\hrulefill\;v_2\;\hrulefill\;}\\
% %             \quad&\quad&\vdots&\quad&\quad     \\
% %             \multicolumn{5}{c}{\;\hrulefill\;v_{n}\;\hrulefill\;}   \\
% %         \end{array}
% % 	\right],	
% % $$
% % 
% % 
% % if $\tilde \cM=\cM[p]$, $p=[a_1^{s_1},a_2^{s_2},\dots,a_r^{s_r}]$, then the $(n+1)\times(d+1)$ matrix that encodes the vertices of $\tilde P$ is the following matrix $\tilde V$
% % 
% % $$
% %       \tilde V = 
% %       \left[
% %       \begin{array}{ccccc|c}
% %             \multicolumn{5}{c|}{\;\hrulefill\;v_1\;\hrulefill\;} &-s1\\
% %             \multicolumn{5}{c|}{\;\hrulefill\;v_2\;\hrulefill\;} &-\delta s_2\\
% %             \multicolumn{5}{c|}{\;\hrulefill\;v_3\;\hrulefill\;} &-\delta^2 s_3\\
% %             \quad&\quad&\vdots&\quad&\quad     &\vdots\\
% %             \multicolumn{5}{c|}{\;\hrulefill\;v_r\;\hrulefill\;} &-\delta^{r-1} s_r\\
% %             \multicolumn{5}{c|}{\;\hrulefill\;v_{r+1}\;\hrulefill\;} &0\\
% %             \quad&\quad&\vdots&\quad&\quad     &\vdots\\
% %             \multicolumn{5}{c|}{\;\hrulefill\;v_{n}\;\hrulefill\;}   &0\\%\cline{1-5}	
% % 	    \multicolumn{5}{c|}{\;\hrulefill\;\veczero\;\hrulefill\;}   &1
% %         \end{array}
% % 	\right].
% % $$
% % 
% % When $\delta$ is small enough, then the vertex figure of $p$ in $\tilde P$ is isomorphic to $P$, hence the face of $\tilde P$ that contain $p$ are isomorphic to pyramids over face of $P$. On the other hand, the faces of $\tilde P$ that do not contain $p$ correspond to faces of a regular triangulation of $P$: a \emph{lexicographic triangulation} of $P$ on $[v_r^{-s_r},\dots,v_2^{-s_2},v_1^{-s_1}]$.
% % 
% % 
% % \begin{figure}[htpb]
% % \begin{center}
% % \includegraphics[width=\textwidth]{Figures/lifting.pdf}
% % \end{center}
% %  \caption{The lifting of a pentagon $P$ to $\tilde P$ when $p=[a_1^-,a_4^+]$, and its upper and lower envelope.}
% %  \label{fig:lifting}
% % \end{figure}
% % 
% % The following exposition is based on~\cite{DeLoeraRambauSantosBOOK}\footnote{The exposition is based on~\cite{DeLoeraRambauSantosBOOK}, however the definition that we use here uses a different ordering, the same as in~\cite{Santos2002}, that mirrors the definition of lexicographic extension.}, and gives a recursive definition in terms of a sequence of operations of pushing and pulling.
% % 
% % \begin{definition}[from~\cite{DeLoeraRambauSantosBOOK}]
% % Let $P$ be a $d$-polytope with $n$ vertices $v_1,\dots,v_n$. The \emph{lexicographic subdivision} of $P$ on $[v_1^{s_1},v_2^{s_2},\dots,v_k^{s_k}]$, where $s_i=\pm 1$, is defined recursively as follows.
% % \begin{itemize}
% %  \item If $s_1=+1$ (pushing), then the lexicographic triangulation of $P$ equals the triangulation obtained as the union of the lexicographic triangulation of $P\setminus v_1$ on $[v_2^{s_2},\dots,v_k^{s_k}]$, and the simplices joining $v_1$ to the (triangulated) faces of $P\setminus v_1$ visible from it.
% %  \item If $s_1=-1$ (pulling), then the lexicographic triangulation of $P$ equals the unique triangulation in which every maximal simplex contains $v_1$ and which, restricted to each proper face $F$ of $P$, coincides with the lexicographic triangulation of that face.
% % \end{itemize}
% % \end{definition}
% 
% % 
% % \section{Comparing the constructions}\label{sec:comparing}
% % In this section we compare the two constructions, which are strongly related. The goal is to prove that all neighborly polytopes in $\cO$ belong to $\cG$. From Proposition~\ref{prop:allquotientsofGalesewnareGalesewn} one deduces that to prove that $\cO\subseteq \cG$ it is enough to see that $\cS\subseteq \cG$. As a first step we will prove that if we sew on a neighborly polytope in $\cG$ (through a specific universal flag), we obtain a new polytope in $\cG$. 
% % 
% % Let $\cP$ be a neighborly matroid in $\cG$. That means that its dual matroid $\cM=\cP^*$ is constructed using Gale sewing as in Section~\ref{sec:thethm}. Specifically, $\cM=\cM_m$ where $\cM_0=\stc{r}$ is the matroid of a simplex $\{a_0,\dots,a_r\}$ containing the origin and
% % % Let $\cM=\cM_m$ be a balanced matroid in $\cG$ constructed as in Section~\ref{sec:thethm}. That is, let $\cM_0=\stc{d}$ be the matroid of a simplex $\{a_0,\dots,a_d\}$ containing the origin. We define 
% % \begin{align*}
% % \cM_k&=\cM_{k-1}[x_k][y_k], 
% % \end{align*}
% % with $x_k$ and $y_k$ being the lexicographic extensions
% % \begin{align*}
% % x_k&=[e_{k1}^{s_{k1}},\dots,e_{kr}^{s_{kr}}],& y_k&=[x_k^-,e_{k1}^{-},\dots,e_{k(r-1)}^{-}].
% % \end{align*}
% % % and the $e_{ij}$ are different elements of $\cM_{i-1}$. 
% % 
% % % Let $\cP=\cM^*$ be the dual matroid of $\cM$. Since $\cM$ is balanced, $\cP$ is neighborly. 
% % Let $T_j=\bigcup_{i=0}^{j-1}(x_{m-i},y_{m-i})$ and let $\cT=\{T_i\}_{i=1}^{m}$. Define $\cP_k=\cM_k^*$, and observe that $\cP_k=\cP_m/T_{m-k}$ for $k=0,\dots,m$. By construction, $\cT$ is a universal flag of $\cP$.
% % 
% % Hence, we can apply the sewing construction of Theorem~\ref{thm:shemersewing} to $\cP$ and $\cT$. Let $\tilde \cP$ be $\cP\cup p$, with $p$ sewn on~$\cP$ through $\cT$. We define $\tilde T_{j+1}=T_{j}\cup y_{m-j}\cup p$, then $\tilde \cT=\{\tilde T_i\}_{i=1}^{m}$ is a universal flag of $\tilde \cP$ by Theorem~\ref{thm:shemersewing}. We denote $\tilde P_k=\tilde P_m/\tilde T_{m-k}$. To provide shorter proofs, we will sometimes refer to $p$ as $x_{m+1}$.
% % 
% % Finally, let $\tilde \cM=\tilde \cM_m$ be the matroid constructed as follows:
% % \begin{align*}
% % \tilde \cM_0&=\stc{r+1} \text{ on a ground set }\{\tilde a_1,\dots,\tilde a_{r+1},\tilde x_1\},\\
% % \tilde y_k&=[\tilde x_k^+,\tilde e_{k1}^{-s_{k1}},\dots,\tilde e_{k(r+1)}^{-s_{k(r+1)}}],& \tilde x_{k+1}&=[\tilde y_k^-,\tilde e_{k1}^{-},\dots,\tilde e_{kr}^{-}],\\
% % \tilde\cM_{k}&=\tilde\cM_{k-1}[\tilde y_k][\tilde x_{k+1}], 
% % \end{align*}
% % where if $e_{ij}=x$ then $\tilde e_{ij}$  means the element labeled as $\tilde x$. 
% % 
% % Then we claim that $\tilde \cM$ is the dual configuration of $\tilde\cP$, and hence $\tilde\cP$ is in $\cG$.
% % 
% % \vspace{.5cm}
% % \begin{figure}[htpb]
% % \begin{center}
% % \includegraphics[width=\textwidth]{Figures/exampleShemervsMe}
% % \end{center}
% %  \caption{Example: $\cM$ is constructed from $\{A,B\}$ after Gale sewing $C=[B^+]$ and $D=[C^-]$. In its dual $\cP=\cM^*$, $\{C,D\}$ is a universal edge. $\tilde \cP=\cP[E]$ is obtained by sewing $E$ on $\cP$. Its dual matroid, $\tilde \cM=\tilde \cP^*$ can be constructed from $\{A,B,C\}$ and Gale sewing $D=[C^+,B^-]$ and $E=[D^-,C^-]$.}
% %  \label{fig:shemervsme}
% % \end{figure}
% % \vspace{.5cm}
% % 
% % \begin{theorem}\label{thm:Mk=Pkstar}
% %  With the notations from above, $\tilde \cM\simeq\tilde\cP^*$
% % via the isomorphism $x\mapsto\tilde x$.
% % \end{theorem}
% % 
% % \begin{proof}
% % We will prove that $\tilde \cM_k\simeq \tilde \cP_k^*$, using Theorem~\ref{thm:minorsfixmatroid} twice. Specifically, we will use that if $\cM\setminus p\simeq \cN\setminus p$ and $\cM/ p\simeq \cN/ p$, then $\cM$ and $\cN$ are the same oriented matroid up to the reorientation of $p$. If additionally there is an element $q$ such that $p$ and $q$ are covariant (or contravariant) in $\cN$ and $\cM$, then $\cM\simeq \cN$.
% % 
% % In particular, we will prove that $\tilde \cM_k/\tilde x_{k+1}\simeq \tilde\cP_k^*/x_{k+1}$ and that $\tilde \cM_k\setminus \tilde x_{k+1}\simeq \tilde\cP_k^*\setminus x_{k+1}$. Then the claim $\tilde \cM\simeq\tilde\cP^*$ will follow directly from the fact that $\tilde x_{k+1}$ and $\tilde y_k$ are covariant in $\tilde\cM_k$ and that $x_{k+1}$ and $y_k$ are covariant in $\tilde\cP_k^*$.
% % 
% % \begin{enumerate}
% %  \item $\tilde \cM_k/\tilde x_{k+1}\simeq \tilde\cP_k^*/x_{k+1}$.
% % 
% %  Since $\tilde\cP_k^*/x_{k+1}=\cP_k^*=\cM_k$, we just need to prove that \begin{equation}\label{eq:quotientsofGaleareShemer}\tilde\cM_k/\tilde x_{k+1}\simeq \cM_k.\end{equation}
% % %  with the natural isomorphism. 
% % Our main tool here is Lemma~\ref{lem:quotientsofGalesewnareGalesewn}. Observe that \begin{displaymath}(\tilde \cM_k/\tilde x_{k+1})\simeq (\tilde \cM_{k-1}/\tilde x_{k})[x'_k][y'_k],\end{displaymath}
% % where $x'_k=[\tilde e_{k1}^{s_{k1}},\dots,\tilde e_{kr}^{s_{kr}}]$ and $y'_{k}=[{x'_k}^-,\tilde e_{k1}^{-},\dots,\tilde e_{k(r-1)}^{-}]$.
% % Using that $\tilde \cM_0/\tilde x_1\simeq \cM_0$ we get the desired result by induction on $k$.
% % 
% %  \item $\tilde \cM_k\setminus \tilde x_{k+1}\simeq \tilde\cP_k^*\setminus x_{k+1}$.
% % 
% % This proof is by induction on $k$ and uses again Theorem~\ref{thm:minorsfixmatroid}. We prove that $\left(\tilde \cM_k\setminus \tilde x_{k+1}\right)\setminus \tilde y_k \simeq \left(\tilde\cP_{k}^*\setminus x_{k+1}\right)\setminus y_k$, and that $\left(\tilde \cM_k\setminus \tilde x_{k+1}\right)/ \tilde y_k \simeq \left(\tilde\cP_{k}^*\setminus x_{k+1}\right)/ y_k$. Now, $\tilde y_k$ is contravariant with $\tilde x_k$ in $\tilde\cM_k$ by construction. And observe that $y_k$ is contravariant with $x_k$ in $\left({\tilde\cP_{k}/ x_{k+1}}\right)^*$ since they are covariant in the primal: by Proposition~\ref{prop:allquotientsofle} $\tilde\cP_{k}/ x_{k+1}\simeq P_{k}/ x_{k}[y_k^-,\dots]$.
% % 
% % By induction hypothesis \begin{displaymath}\left(\tilde \cM_k\setminus \tilde x_{k+1}\right)\setminus \tilde y_k =\tilde \cM_{k-1}\simeq{\tilde\cP_{k-1}}^*=\left({\tilde\cP_{k}/\{y_k,x_{k+1}\}}\right)^*=\left(\tilde\cP_{k}^*\setminus x_{k+1}\right)\setminus y_k.\end{displaymath}
% % 
% %  Hence, it only remains to check that $\left(\tilde \cM_k\setminus \tilde x_{k+1}\right)/\tilde y_k\simeq \left(\tilde \cP_k\setminus x_{k+1}\right)/y_k$. 
% % 
% % Using Lemma~\ref{lem:contractdeletele} and \eqref{eq:quotientsofGaleareShemer},
% %  \begin{displaymath}\left(\tilde \cM_k\setminus \tilde x_{k+1}\right)/\tilde y_k\simeq\left(\tilde \cM_k / \tilde x_{k+1}\right)\setminus \tilde y_k\simeq \cM_k\setminus y_k.\end{displaymath}
% % 
% % And using again Lemma~\ref{lem:contractdeletele},
% % \begin{displaymath} \left(\tilde\cP_k^*\setminus x_{k+1}\right)/y_k=\left({\tilde\cP_k/x_{k+1}\setminus y_k}\right)^*\simeq\left({\tilde \cP_k\setminus x_{k+1}/ y_k}\right)^*=\left({\cP_k/ y_k}\right)^*={\cP_k}^*\setminus y_k.\end{displaymath}
% % 
% % Now the result follows since $\cM_k=\cP_k^*$ by definition.
% % \end{enumerate}
% % % 
% % % First, we prove that \begin{equation}\label{eq:quotientsofGaleareShemer}\tilde\cM_k/\tilde x_{k+1}\simeq \cM_k\end{equation} with the natural isomorphism. Since $\cM_k=\cP_k^*=\tilde\cP_k^*/x_{k+1}$, we will have the first part of the proof.
% % % 
% % % Our main tool here is Lemma~\ref{lem:quotientsofGalesewnareGalesewn}. Observe that $$(\tilde \cM_k/\tilde x_{k+1})\simeq (\tilde \cM_{k-1}/\tilde x_{k})[x'_k][y'_k],$$
% % % where $x'_k=[\tilde e_{k1}^{s_{k1}},\dots,\tilde e_{k(d+1)}^{s_{k(d+1)}}]$ and $y'_{k}=[{x'_k}^-,\tilde e_{k1}^{-},\dots,\tilde e_{k{d-1}}^{-}]$.
% % % Using that $\tilde \cM_0/\tilde x_1\simeq \cM_0$ we get the desired result by induction on $k$. 
% % % 
% % % The second step is to prove that  $$\tilde \cM_k\setminus \tilde x_{k+1}\simeq \tilde\cP_k^*\setminus x_{k+1}.$$ 
% % % 
% % % This proof uses again Theorem~\ref{thm:minorsfixmatroid} and induction on $k$. We prove that $\left(\tilde \cM_k\setminus \tilde x_{k+1}\right)\setminus \tilde y_k \simeq \left(\tilde\cP_{k}^*\setminus x_{k+1}\right)\setminus y_k$, and that $\left(\tilde \cM_k\setminus \tilde x_{k+1}\right)/ \tilde y_k \simeq \left(\tilde\cP_{k}^*\setminus x_{k+1}\right)/ y_k$. Now, $\tilde y_k$ is contravariant with $\tilde x_k$ in $\tilde\cM_k$ by construction. And observe that $y_k$ is contravariant with $x_k$ in $\left({\tilde\cP_{k}/ x_{k+1}}\right)^*$ since they are covariant in the primal: by Proposition~\ref{prop:allquotientsofle} $\tilde\cP_{k}/ x_{k+1}\simeq P_{k}/ x_{k}[y_k^-,\dots]$.
% % % 
% % % By induction hypothesis $$\left(\tilde \cM_k\setminus \tilde x_{k+1}\right)\setminus \tilde y_k =\tilde \cM_{k-1}\simeq{\tilde\cP_{k-1}}^*=\left({\tilde\cP_{k}/\{y_k,x_{k+1}\}}\right)^*=\left(\tilde\cP_{k}^*\setminus x_{k+1}\right)\setminus y_k.$$
% % % 
% % % %  Now, $\tilde y_k$ is contravariant with $\tilde x_k$ in $\tilde\cM_k$ by construction. And observe that $y_k$ is contravariant with $x_k$ in $\left({\tilde\cP_{k}/ x_{k+1}}\right)^*$ since they are covariant in the primal: by Proposition~\ref{prop:allquotientsofle} $\tilde\cP_{k}/ x_{k+1}\simeq P_{k}/ x_{k}[y_k^-,\dots]$.
% % % 
% % %  Hence, it only remains to check that $\left(\tilde \cM_k\setminus \tilde x_{k+1}\right)/\tilde y_k\simeq \left(\tilde \cP_k\setminus x_{k+1}\right)/y_k$. 
% % % 
% % % Using Lemma~\ref{lem:contractdeletele} and \eqref{eq:quotientsofGaleareShemer},
% % %  $$\left(\tilde \cM_k\setminus \tilde x_{k+1}\right)/\tilde y_k\simeq\left(\tilde \cM_k / \tilde x_{k+1}\right)\setminus \tilde y_k\simeq \cM_k\setminus y_k.$$
% % % 
% % % And using again Lemma~\ref{lem:contractdeletele},
% % % $$ \left(\tilde\cP_k^*\setminus x_{k+1}\right)/y_k=\left({\left(\tilde\cP_k/x_{k+1}\right)\setminus y_k}\right)^*\simeq\left({\left(\tilde \cP_k\setminus x_{k+1}\right)/ y_k}\right)^*=\left({\cP_k/ y_k}\right)^*={\cP_k}^*\setminus y_k.$$
% % % 
% % % Now the result follows since $\cM_k=\cP_k^*$ by definition.
% % 
% % \end{proof}
% % 
% % There are two missing details to conclude that $\cS\subseteq \cG$ from Theorem~\ref{thm:Mk=Pkstar}:
% % \begin{enumerate}[i)]
% %  \item We have to check that cyclic polytopes are in $\cG$ and that the universal flags of Example~\ref{ex:universalflagsofcyclic} are of the form $T_j=\cup_{i=0}^{j-1}(x_{m-i},y_{m-i})$.
% %  \item We have to check that after a regular sewing, all the flags of Point~\eqref{it:newunifaces} in Theorem~\ref{thm:shemersewing} are also of the form $T_j=\cup_{i=0}^{j-1}(x_{m-i},y_{m-i})$.
% % \end{enumerate}
% % 
% % For the first point, Proposition~\ref{prop:cyclicaregalesewn} tells us that $\cyc{2m}{n}\in \cG$. However, we need to see that we can construct their dual in the order given by any of the universal flags of Example~\ref{ex:universalflagsofcyclic}. But this is a direct consequence of Proposition~\ref{prop:cyclicaregalesewn} and the fact that the automorphism group of $\cyc{2m}{n}$ contains the dihedral group 
% % % (if $n\geq 2m+3$ then it is the dihedral group)~\cite{AltshulerPerles1980}.
% % (see~\cite{AltshulerPerles1980}).
% % Specifically, there is an automorphism that sends $(x_k,y_k)$ to $(s_{n-1},s_{n})$. From Proposition~\ref{prop:cyclicaregalesewn}, we know that these two points are Gale sewn. Now $\cyc{2m}{n}/(x_k,y_k)\simeq \cyc{2m-2}{n-2}$, and the result follows inductively.
% % 
% % The second point is direct: using Lemma~\ref{lem:galesewingorder} we can change the roles of $x_i$ and $y_i$ in the construction of $\cM$. Hence we can change the order of the sewings in $\tilde\cM$. This leads to defining $\tilde T_{j+1}=T_{j}\cup y_{m-j}\cup p$ or as $\tilde T_{j+1}=T_{j}\cup x_{m-j}\cup p$, which provides all the different universal flags of $\tilde \cP$ in Theorem~\ref{thm:shemersewing}. 
% % 
% % \begin{remark}
% % The fact that $\cS\subsetneq\cG$ implies that in some sense Gale sewing generalizes the ordinary sewing. However, it is not true that Theorem~\ref{thm:shemersewing} is a consequence of Theorem~\ref{thm:thethm}. There could be universal flags that are not of the form $T_j=\cup_{i=0}^{j-1}(x_{m-i},y_{m-i})$, and hence that cannot be treated with Theorem~\ref{thm:Mk=Pkstar}.
% % \end{remark}
% 
% 
% \section{Comparing and combining the constructions}\label{sec:comparing}
% In this section we compare and combine the two constructions, which are strongly related. The first goal is to prove that all neighborly polytopes in $\cO$ belong to $\cG$. From Proposition~\ref{prop:allquotientsofGalesewnareGalesewn} one deduces that to prove that $\cO\subseteq \cG$ it is enough to see that $\cE\subseteq \cG$. As a first step we will prove that if we sew on a neighborly polytope in $\cG$ (through a specific universal flag), we obtain a new polytope in $\cG$. 
% 
% Let $\cP$ be a neighborly matroid in $\cG$. That means that its dual matroid $\cM=\cP^*$ is constructed using Gale sewing as in Section~\ref{sec:thethm}. Specifically, $\cM=\cM_m$ where $\cM_0=\stc{r}$ is a minimal totally cyclic configuration $\{a_0,\dots,a_r\}$ of rank $r$ and
% % Let $\cM=\cM_m$ be a balanced matroid in $\cG$ constructed as in Section~\ref{sec:thethm}. That is, let $\cM_0=\stc{d}$ be the matroid of a simplex $\{a_0,\dots,a_d\}$ containing the origin. We define 
% \begin{align*}
% \cM_k&=\cM_{k-1}[x_k][y_k], 
% \end{align*}
% with $x_k$ and $y_k$ being the lexicographic extensions
% \begin{align*}
% x_k&=[e_{k1}^{s_{k1}},\dots,e_{kr}^{s_{kr}}],& y_k&=[x_k^-,e_{k1}^{-},\dots,e_{k(r-1)}^{-}].
% \end{align*}
% % and the $e_{ij}$ are different elements of $\cM_{i-1}$. 
% 
% % Let $\cP=\cM^*$ be the dual matroid of $\cM$. Since $\cM$ is balanced, $\cP$ is neighborly. 
% Let $T_j=\bigcup_{i=0}^{j-1} \{x_{m-i},y_{m-i}\}$, that is $T_{m-k}=\{x_m,y_m,\dots,x_{k+1},y_{k+1}\}$. And let $\cT=\{T_i\}_{i=1}^{m}$. 
% Define $\cP_k=\cM_k^*$, and observe that $\cP_k=\cP/T_{m-k}$ for $k=0,\dots,m$. By construction, $\cT$ is a universal flag of $\cP$.
% Let $\cT'$ be some flag that contains $\cT$. Thanks to Lemma~\ref{lem:galesewingorder} we can assume without loss of generality that all split faces in $\cT'$ are $y$-split.
% 
% We can apply the extended sewing construction of Theorem~\ref{thm:extshemersewing} to $\cP$ and $\cT'$. Let $\tilde \cP$ be $\cP\cup p$, with $p$ sewn onto~$\cP$ through $\cT'$. We define $\tilde T_{j+1}=T_{j}\cup y_{m-j}\cup p$, that is $\tilde T_{m-k}=\{x_m,y_m,\dots,x_{k+2},y_{k+2}\}\cup\{y_{k+1}\}\cup\{p\}$.	
% Then $\tilde \cT=\{\tilde T_i\}_{i=1}^{m}$ is a universal flag of $\tilde \cP$ by Proposition~\ref{prop:extnewunifaces}. We denote $\tilde \cP_k=\tilde \cP/\tilde T_{m-k}$ and observe that $\tilde \cP_k\simeq \cP_k[\cT'/T_{m-k}]$ where the sewn vertex is $x_{k+1}$, and thus
% $\tilde \cP_k\setminus x_{k+1}\simeq \cP_k$. To provide shorter proofs, we will sometimes refer to $p$ as $x_{m+1}$.
% 
% Finally, let $\tilde \cM=\tilde \cM_m$ be the oriented matroid constructed as follows:
% \begin{align*}
% \tilde \cM_0&=\stc{r+1} \text{ on a ground set }\{\tilde a_1,\dots,\tilde a_{r+1},\tilde x_1\},\\
% \tilde y_k&=
% \begin{cases} [\tilde x_k^+,{(\tilde e_{k1})}^{-s_{k1}},\dots,{(\tilde e_{kr})}^{-s_{kr}}]& \text{if $T_{m-k+1}$ is not split in $\cT'$,}\\
% [\tilde x_k^-,{(\tilde e_{k1})}^{s_{k1}},\dots, {(\tilde e_{kr})}^{s_{kr}}]& \text{if $T_{m-k+1}$ is split in $\cT'$.}
% \end{cases}\\
% % [\tilde x_k^+,\tilde e_{k1}^{-s_{k1}},\dots,\tilde e_{k(r+1)}^{-s_{k(r+1)}}],&
%  \tilde x_{k+1}&=[\tilde y_k^-,{(\tilde e_{k1})}^{-},\dots,{(\tilde e_{k(r-1)})}^{-}],\\
%  \tilde\cM_{k}&=\tilde\cM_{k-1}[\tilde y_k][\tilde x_{k+1}], 
% \end{align*}
% where if $e_{ij}=x$ then $\tilde e_{ij}$  means the element labeled as $\tilde x$. 
% 
% Then we claim that $\tilde \cM$ is the dual configuration of $\tilde\cP$, and hence $\tilde\cP$ is in $\cG$.
% 
% % \vspace{.5cm}
% \begin{figure}[htpb]
% \begin{center}
% \includegraphics[width=\textwidth]{Figures/exampleShemervsMe}
% \end{center}
%  \caption[Primal and dual sewing]{Example: $\cM$ is constructed from $\{A,B\}$ after Gale sewing $C=[B^+]$ and $D=[C^-]$. In its dual $\cP=\cM^*$, $\{C,D\}$ is a universal edge. $\tilde \cP=\cP[E]$ is obtained by sewing $E$ on $\cP$ through $\{C,D\}$. Its dual matroid, $\tilde \cM=\tilde \cP^*$ can be constructed from $\{A,B,C\}$ and Gale sewing $D=[C^+,B^-]$ and $E=[D^-,C^-]$.}
%  \label{fig:shemervsme}
% \end{figure}
% % \vspace{.5cm}
% 
% \begin{proposition}\label{prop:Mk=Pkstar}
%  With the notations from above, $\tilde \cM\simeq\tilde\cP^*$
% via the isomorphism $x\mapsto\tilde x$.
% \end{proposition}
% 
% \begin{proof}
% We will prove that $\tilde \cM_k\simeq \tilde \cP_k^*$, for all $k$. The proof will use induction on $k$ and assume that $\tilde \cM_{k-1}\simeq{\tilde\cP_{k-1}}^*$. It is straightforward that $\tilde \cM_{0}\simeq{\tilde\cP_{0}}^*$ since $\cP_{0}$ is $0$-dimensional.
% 
% We will use Theorem~\ref{thm:minorsfixmatroid} twice. Specifically, we will use that if $\cM\setminus p\simeq \cN\setminus p$ and $\cM/ p\simeq \cN/ p$, then $\cM$ and $\cN$ are the same oriented matroid up to the reorientation of $p$. If additionally there is an element $q$ such that $p$ and $q$ are covariant (or contravariant) in $\cN$ and $\cM$, then $\cM\simeq \cN$.
% 
% In particular, we will prove that $\tilde \cM_k/\tilde x_{k+1}\simeq \tilde\cP_k^*/x_{k+1}$ and that $\tilde \cM_k\setminus \tilde x_{k+1}\simeq \tilde\cP_k^*\setminus x_{k+1}$. Then the claim $\tilde \cM\simeq\tilde\cP^*$ will follow directly from the fact that $\tilde x_{k+1}$ and $\tilde y_k$ are covariant in $\tilde\cM_k$ and that $x_{k+1}$ and $y_k$ are covariant in $\tilde\cP_k^*$.
% 
% 
% % \begin{enumerate}
% %  \item 
% \medskip
% \noindent \underline{$\tilde \cM_k/\tilde x_{k+1}\simeq \tilde\cP_k^*/x_{k+1}$}
% 
%  Since $\tilde\cP_k^*/x_{k+1}\simeq\cP_k^*=\cM_k$ because $\tilde\cP_k\setminus x_{k+1}\simeq\cP_k$, we just need to prove that \begin{equation}\label{eq:quotientsofGaleareShemer}\tilde\cM_k/\tilde x_{k+1}\simeq \cM_k.\end{equation}
% %  with the natural isomorphism. 
% By Lemma~\ref{lem:quotientsofGalesewnareGalesewn}, \((\tilde \cM_k/\tilde x_{k+1})\simeq (\tilde \cM_{k-1}/\tilde x_{k})[x'_k][y'_k],\)
% where $x'_k=[\tilde e_{k1}^{s_{k1}},\dots,\tilde e_{kr}^{s_{kr}}]$ and $y'_{k}=[{x'_k}^-,\tilde e_{k1}^{-},\dots,\tilde e_{k(r-1)}^{-}]$.
% Using that $\tilde \cM_0/\tilde x_1\simeq \cM_0$ we get the desired result by induction on $k$.
% 
% %  \item 
% \medskip
% \noindent \underline{$\tilde \cM_k\setminus \tilde x_{k+1}\simeq \tilde\cP_k^*\setminus x_{k+1}$}
% 
% The first step is to prove that $(\tilde \cM_k\setminus \tilde x_{k+1})\setminus \tilde y_k \simeq (\tilde\cP_{k}^*\setminus x_{k+1})\setminus y_k$.
% Indeed, using the induction hypothesis,\[(\tilde \cM_k\setminus \tilde x_{k+1})\setminus \tilde y_k =\tilde \cM_{k-1}\simeq{\tilde\cP_{k-1}}^*=({\tilde\cP_{k}/\{y_k,x_{k+1}\}})^*=(\tilde\cP_{k}^*\setminus x_{k+1})\setminus y_k.\]
% 
% Now we prove that $(\tilde \cM_k\setminus \tilde x_{k+1})/ \tilde y_k \simeq (\tilde\cP_{k}^*\setminus x_{k+1})/ y_k$. 
% First, using Lemma~\ref{lem:contractdeletele} and \eqref{eq:quotientsofGaleareShemer}, we see that
%  \begin{displaymath}(\tilde \cM_k\setminus \tilde x_{k+1})/\tilde y_k\simeq(\tilde \cM_k / \tilde x_{k+1})\setminus \tilde y_k\simeq \cM_k\setminus y_k.\end{displaymath}
% Now, using again Lemma~\ref{lem:contractdeletele} and that $\tilde \cP_k\setminus x_{k+1}\simeq \cP_k$, we see that
% \begin{displaymath} (\tilde\cP_k^*\setminus x_{k+1})/y_k=({\tilde\cP_k/x_{k+1}\setminus y_k})^*\simeq({\tilde \cP_k\setminus x_{k+1}/ y_k})^*=({\cP_k/ y_k})^*={\cP_k}^*\setminus y_k.\end{displaymath}
% Our claim follows since $\cM_k=\cP_k^*$ by definition.
% 
% \smallskip
% Because of Theorem~\ref{thm:minorsfixmatroid}, so far we have seen that $\tilde \cM_k\setminus \tilde x_{k+1}\simeq \tilde\cP_k^*\setminus x_{k+1}$ up to reorientation of $y_k$. We will conclude the proof by seeing that $y_k$ and $\tilde y_k$ have the same orientation in $\cM_k$ and in $\tilde \cM_k$ respectively.
% 
% If $T_{m-k+1}$ is not split, then $\tilde y_k$ is contravariant with $\tilde x_k$ in $\tilde\cM_k$ by construction. Moreover, $y_k$ is contravariant with $x_k$ in $({\tilde\cP_{k}/ x_{k+1}})^*$ since they are covariant in the primal: by Proposition~\ref{prop:allquotientsofle} \[\tilde\cP_{k}/ x_{k+1}\simeq\big(\cP_{k}\underbrace{[\cT'/T_{m-k}]}_{x_{k+1}}\big)/x_{k+1}\simeq \big(\cP_{k}/ x_{k}\big)\underbrace{[y_k^-,\dots]}_{x_k},\]
% where the last isomorphism sends $x_k$ to the sewn vertex, which is $(+1)$-inseparable from $y_k$.
% 
% If $T_{m-k+1}$ is split, then $\tilde y_k$ is covariant with $\tilde x_k$ in $\tilde\cM_k$. Moreover, $y_k$ is covariant with $x_k$ in $({\tilde\cP_{k}/ x_{k+1}})^*$ because $\tilde\cP_{k}/ x_{k+1}\simeq \cP_{k}/ x_{k}[y_k^+,\dots]$. 
% % \end{enumerate}
% 
% \end{proof}
% 
% % 
% % There are two missing details to conclude that $\cS\subseteq \cG$ from Theorem~\ref{thm:Mk=Pkstar}:
% % \begin{enumerate}[i)]
% %  \item We have to check that cyclic polytopes are in $\cG$ and that the universal flags of Example~\ref{ex:universalflagsofcyclic} are of the form $T_j=\cup_{i=0}^{j-1}(x_{m-i},y_{m-i})$.
% %  \item We have to check that after a regular sewing, all the flags of Point~\eqref{it:newunifaces} in Theorem~\ref{thm:shemersewing} are also of the form $T_j=\cup_{i=0}^{j-1}(x_{m-i},y_{m-i})$.
% % \end{enumerate}
% % 
% % For the first point, Proposition~\ref{prop:cyclicaregalesewn} tells us that $\cyc{2m}{n}\in \cG$. However, we need to see that we can construct their dual in the order given by any of the universal flags of Example~\ref{ex:universalflagsofcyclic}. But this is a direct consequence of Proposition~\ref{prop:cyclicaregalesewn} and the fact that the automorphism group of $\cyc{2m}{n}$ contains the dihedral group 
% % % (if $n\geq 2m+3$ then it is the dihedral group)~\cite{AltshulerPerles1980}.
% % (see~\cite{AltshulerPerles1980}).
% % Specifically, there is an automorphism that sends $(x_k,y_k)$ to $(s_{n-1},s_{n})$. From Proposition~\ref{prop:cyclicaregalesewn}, we know that these two points are Gale sewn. Now $\cyc{2m}{n}/(x_k,y_k)\simeq \cyc{2m-2}{n-2}$, and the result follows inductively.
% % 
% % The second point is direct: using Lemma~\ref{lem:galesewingorder} we can change the roles of $x_i$ and $y_i$ in the construction of $\cM$. Hence we can change the order of the sewings in $\tilde\cM$. This leads to defining $\tilde T_{j+1}=T_{j}\cup y_{m-j}\cup p$ or as $\tilde T_{j+1}=T_{j}\cup x_{m-j}\cup p$, which provides all the different universal flags of $\tilde \cP$ in Theorem~\ref{thm:shemersewing}. 
% 
% There is a missing detail to conclude that $\cE\subseteq \cG$ from Proposition~\ref{prop:Mk=Pkstar}:
% we have to check that after sewing, the universal flags of Proposition~\ref{prop:extnewunifaces} are also of the form $T_j=\cup_{i=0}^{j-1}(x_{m-i},y_{m-i})$ for some Gale sewn configuration.
% 
% This is consequence of Lemma~\ref{lem:galesewingorder}, which allows to change the order of the sewings in $\tilde\cM$.
% 
% \begin{remark}
% The fact that $\cE\subsetneq\cG$ implies that in some sense Gale sewing generalizes ordinary sewing. However, it is not true that Theorem~\ref{thm:shemersewing} is a consequence of Theorem~\ref{thm:thethm}, because there are neighborly matroids that have universal flags but are not in $\cG$. Hence one can sew on them but they 
% % There could be universal flags that are not of the form $T_j=\cup_{i=0}^{j-1}(x_{m-i},y_{m-i})$, and hence that 
% cannot be treated with Proposition~\ref{prop:Mk=Pkstar}. 
% This will become clear in Section~\ref{sec:nonrealizable}, where both constructions are needed.
% \end{remark}
% 
% 
% 
% \subsection{Some exact numbers}
% 
% Fix $n$ and $d=2m$. We have worked with four families of neighborly $d$-polytopes with $n$ vertices:
% \begin{description}
%  \item[$\cN$:] All neighborly $d$-polytopes with $n$ vertices.
%  \item[$\cG$:] All Gale sewn $d$-polytopes with $n$ vertices.
%  \item[$\cS$:] All totally sewn $d$-polytopes with $n$ vertices.
%  \item[$\cE$:] All $d$-polytopes with $n$ vertices obtained with the extended sewing construction.
%  \item[$\cO$:] All $d$-polytopes with $n$ vertices obtained by extended sewing and omitting.
% \end{description}
% 
% % We know that the first inclusion is strict. For example, there are 13 neighborly $6$-polytopes with $10$ vertices that can be obtained from $\cyc{6}{9}$ by double sewing and omitting a vertex, but not directly by sewing~\cite{Shemer1982}.
% 
% % We also know that $\cG\neq \cN$. In particular, in \cite{BokowskiSturmfels1987} the sphere ``$ M^{10}_{416}$'' is proved to be polytopal, giving an example of a neighborly $4$-polytope with $10$ vertices that has no inseparable pair. All polytopes in $\cG$ have inseparable pairs.
% 
% Table~\ref{tb:numcombtypes} contains the exact number of combinatorial types in each of these families for the cases $d=4$ and $n=8,9$ and for $d=6$ and $n=10$. Exact numbers for $\cN$ come from~\cite{GruenbaumSreedharan1967}, \cite{AltshulerSteinberg1973} and~\cite{BokowskiShemer1987}, exact numbers for $\cS$ and $\cO$ come from~\cite{Shemer1982}. Numbers for $\cG$ and $\cE$ have been computed with the help of \texttt{polymake}~\cite{polymake}.
% 
% \begin{table}[htpb]
% \centering
%   \caption{Exact number of combinatorial types}	\label{tb:numcombtypes}
%   \setlength{\tabcolsep}{10pt}
% %   \renewcommand{\arraystretch}{1.2}
% % \begin{center}
%   \begin{tabular}{| c | c || c | c | c | c | c |}
%     \hline
%       $d$& $n$ & $\cS$ & $\cE$ & $\cO$ & $\cG$ & $\cN$\\
%     \hline \hline 
% %       2 & $n$ & 1 & 1 & 1 & 1 & 1\\ 
% %     \hline
% %       $2d$ & $\leq 2d+3$ & 1 & 1 & 1 & 1 & 1\\ 
% %     \hline
%       4 & 8 & 3 & 3 & 3 & 3 & 3 \\ 
% %     \hline
%       4 & 9 & 18 & 18 & 18 & 18 & 23 \\ 
% %     \hline
%       6 & 10 & 15 & 26 & 28 & 28 & 37 \\ 
%     \hline
%   \end{tabular}
% % \end{center}
% \end{table}
% 
% 
% In view of Table~\ref{tb:numcombtypes}, the relationships that we know between these families are summarized in the following proposition.
% \begin{proposition}
% \(\cS\subsetneq\cE\subsetneq\cO\subseteq\cG\subsetneq\cN.\)
% \end{proposition}
% 
% Which yields the following question.
% \begin{question}
% Is $\cO=\cG$?
% \end{question}
% 
% 
% % 
% % In \cite{BokowskiSturmfels1987} the sphere ``$ M^{10}_{416}$'' is proved to be polytopal, giving an example of a neighborly $4$-polytope with $10$ vertices that has no inseparable pair. In particular, there are neighborly polytopes with no universal edges. This implies that there are neighborly polytopes that cannot be constructed iteratively using balanced matroids.
% % 
% % Another issue is how big these families are. In~\cite{Shemer1982} it is proven that $|\cS|\geq 2^{c_d n\log n}$. How bigger is $\cG$?
% 
% 
% 
% 
% \subsection{Non-realizable neighborly oriented matroids}\label{sec:nonrealizable}
% Since the only neighborly matroids of rank~$3$ are cyclic polytopes, there are no non-realizable neighborly matroids of rank~$3$. However, the sphere ``$M^{10}_{425}$'' from Altshuler's list~\cite{Altshuler1977} corresponds to a neighborly matroid of rank $5$ with $10$ elements. In~\cite{BokowskiGarms1987}, this matroid is proved to be non-realizable, giving a proof that there exist non-realizable neighborly matroids. Kortenkamp's construction~\cite{Kortenkamp1997} can be used to build non-realizable neighborly matroids of corank $3$. We show that there are many non-realizable neighborly matroids.
% 
% \begin{theorem}\label{thm:nonrealizable}
%  There exists a non-realizable neighborly matroid of rank $d$ with $n$ elements for every $d\geq 5$ and $n\geq d+5$.
% \end{theorem}
% 
% 
% % Table~\ref{tb:facetsM425} contains a list of the facets of $M^{10}_{425}$.
% % 
% % \begin{table}
% % \begin{tabular}{ccccccccccc}
% % 0123&
% % 0167&
% % 0456&
% % 1269&
% % 2345&
% % 2458&
% % 4567&
% % 0126&
% % 0179&
% % 0467\\
% % 1345&
% % 2348&
% % 2578&
% % 4579&
% % 0135&
% % 0189&
% % 0479&
% % 1348&
% % 2357&
% % 2678\\
% % 4589&
% % 0145&
% % 0236&
% % 0489&
% % 1389&
% % 2367&
% % 2689&
% % 5789&
% % 0148&
% % 0356\\
% % 1239&
% % 1679&
% % 2389&
% % 3567&
% % 6789&
% % \end{tabular}
% % \caption{List of facets of $M^{10}_{425}$.}\label{tb:facetsM425}
% % \end{table}
% \begin{proof}
% 
% We start with $M^{10}_{425}$. With the vertex labeling of \cite{Altshuler1977}, $\{0,1\}$, $\{2,3\}$, $\{4,5\}$, $\{6,7\}$ and $\{8,9\}$ are universal edges of $M^{10}_{425}$ because the corresponding contractions are polygons with $8$ vertices. In particular, $\{0,1\}\subset \{0,1,2,3\}$ is a universal flag. Hence, applying Theorem~\ref{thm:extshemersewing} we get many non-realizable matroids of rank $5$ with $n$ vertices for any $n\geq 10$.
% 
% Now, applying Corollary~\ref{cor:primalGaleSewing} to these matroids, we get non-realizable oriented matroids of rank $5+2k$ and $n$ vertices for any $k\geq 0$ and any $n\geq 10+2k$.
% 
% To get non-realizable matroids of even rank, just observe that any single element extension on the dual of a neighborly matroid of rank $2k+1$ yields the dual of a neighborly matroid of rank $2k+2$.
% \end{proof}
% 
% 
% All neighborly matroids of rank $2m+1$ that have $n\leq2m+3$ vertices are cyclic polytopes. Moreover, all oriented matroids of rank $5$ with $8$ elements are realizable~\cite[Corollary 8.3.3]{OrientedMatroids1993}. Hence the first case that Theorem~\ref{thm:nonrealizable} does not deal with are neighborly matroids of rank $5$ with $9$ elements.
% 
% \begin{question}
%  Do there exist non-realizable neighborly oriented matroids of rank $5$ on $9$ elements?
% \end{question}

% \thispagestyle{empty}
\chapter{The number of neighborly polytopes}\label{ch:counting}


\subsection{Some exact numbers}

Fix $n$ and $d=2m$. We have worked with four families of neighborly $d$-polytopes with $n$ vertices:
\begin{description}
 \item[$\cN$:] All neighborly $d$-polytopes with $n$ vertices.
 \item[$\cG$:] All Gale sewn $d$-polytopes with $n$ vertices.
 \item[$\cS$:] All totally sewn $d$-polytopes with $n$ vertices.
 \item[$\cE$:] All $d$-polytopes with $n$ vertices obtained with the extended sewing construction.
 \item[$\cO$:] All $d$-polytopes with $n$ vertices obtained by extended sewing and omitting.
\end{description}

% We know that the first inclusion is strict. For example, there are 13 neighborly $6$-polytopes with $10$ vertices that can be obtained from $\cyc{6}{9}$ by double sewing and omitting a vertex, but not directly by sewing~\cite{Shemer1982}.

% We also know that $\cG\neq \cN$. In particular, in \cite{BokowskiSturmfels1987} the sphere ``$ M^{10}_{416}$'' is proved to be polytopal, giving an example of a neighborly $4$-polytope with $10$ vertices that has no inseparable pair. All polytopes in $\cG$ have inseparable pairs.

Table~\ref{tb:numcombtypes} contains the exact number of combinatorial types in each of these families for the cases $d=4$ and $n=8,9$ and for $d=6$ and $n=10$. Exact numbers for $\cN$ come from~\cite{GruenbaumSreedharan1967}, \cite{AltshulerSteinberg1973} and~\cite{BokowskiShemer1987}, exact numbers for $\cS$ and $\cO$ come from~\cite{Shemer1982}. Numbers for $\cG$ and $\cE$ have been computed with the help of \texttt{polymake}~\cite{polymake}.

\begin{table}[htpb]
\centering
  \caption{Exact number of combinatorial types}	\label{tb:numcombtypes}
  \setlength{\tabcolsep}{10pt}
%   \renewcommand{\arraystretch}{1.2}
% \begin{center}
  \begin{tabular}{| c | c || c | c | c | c | c |}
    \hline
      $d$& $n$ & $\cS$ & $\cE$ & $\cO$ & $\cG$ & $\cN$\\
    \hline \hline 
%       2 & $n$ & 1 & 1 & 1 & 1 & 1\\ 
%     \hline
%       $2d$ & $\leq 2d+3$ & 1 & 1 & 1 & 1 & 1\\ 
%     \hline
      4 & 8 & 3 & 3 & 3 & 3 & 3 \\ 
%     \hline
      4 & 9 & 18 & 18 & 18 & 18 & 23 \\ 
%     \hline
      6 & 10 & 15 & 26 & 28 & 28 & 37 \\ 
    \hline
  \end{tabular}
% \end{center}
\end{table}


In view of Table~\ref{tb:numcombtypes}, the relationships that we know between these families are summarized in the following proposition.
\begin{proposition}
\(\cS\subsetneq\cE\subsetneq\cO\subseteq\cG\subsetneq\cN.\)
\end{proposition}

Which yields the following question.
\begin{question}
Is $\cO=\cG$?
\end{question}


% 
% In \cite{BokowskiSturmfels1987} the sphere ``$ M^{10}_{416}$'' is proved to be polytopal, giving an example of a neighborly $4$-polytope with $10$ vertices that has no inseparable pair. In particular, there are neighborly polytopes with no universal edges. This implies that there are neighborly polytopes that cannot be constructed iteratively using balanced matroids.
% 
% Another issue is how big these families are. In~\cite{Shemer1982} it is proven that $|\cS|\geq 2^{c_d n\log n}$. How bigger is $\cG$?


\section{Bounds on the number of neighborly polytopes}\label{sec:counting}

The aim of this section is to find lower bounds for $\lnei{n}{d}$, the number of combinatorial types of vertex-labeled neighborly polytopes with $n$ vertices in dimension~$d$. 
Because of Theorem~\ref{thm:neigharerigid}, two neighborly polytopes with the same combinatorial type have the same oriented matroid. Therefore, it is enough to focus on giving bounds for the numbers of labeled realizable neighborly matroids. In the remainder of this paper, all polytopes and oriented matroids will be labeled. Our bounds will be so large that the naive bounds for unlabeled combinatorial types obtained by dividing by $n!$ would have similar asymptotics.

% We will use the Gale sewing technique of Theorem~\ref{thm:thethm} to give bounds for the number of combinatorial types of vertex-labeled polytopes with $n$ vertices in dimension $d$ that are in $\cG$. 
More precisely, we will use the Gale sewing technique of Theorem~\ref{thm:thethm} to give lower bounds on the number of $d$-polytopes with $n$ vertices that are in $\cG$. 
 
A first step is to compute lower bounds for $\lle{n}{r}$, the smallest number of different labeled lexicographic extensions that a balanced matroid of rank $r$ with $n$ elements can have. 
There are $2^{r}\frac{n!}{(n-r)!}$ different expressions for lexicographic extensions of a matroid $\cM$ of rank $r$ and $n$ elements, yet not all of them represent different labeled oriented matroids. We aim to avoid counting the same extension twice with two different expressions. 

\begin{proposition}\label{prop:lble}
 Let $\cM$ be a rank $r$ labeled balanced matroid with $n=r+1+2m$ elements. The number of different labeled lexicographic extensions of $\cM$ fulfills \begin{equation}\label{eq:bndle1}\lle{n}{r}\geq2\cdot\frac{n!}{(n-r+1)!}.%=2\ffp{n}{r-1}.
\end{equation}
\end{proposition}
\begin{proof}
We focus only on those extensions where $s_i=+$ for all $i$. Those are unambiguous except for the last element $a_r^{s_r}$. 

For this, observe that if $[a_1^{+},\dots,a_r^{+}]$ and $[{a'_1}^{+},\dots,{a'_r}^{+}]$, with $r>1$, provide the same oriented matroid, then $a_1$ and $a'_1$ must be contravariant. But balanced matroids of rank $r\geq 2$ and $r+1+2m$ elements only have covariant pairs (see Lemma~\ref{lem:balonlycovar}).
If $a_i$ and $a_i'$ are the first different elements and $i<r$, we can apply the previous argument on the contraction by $\{a_1,\dots,a_{i-1}\}$.

For the last element, observe that $\cM/\{a_1,\dots,a_{r-1}\}$ is a matroid of rank $1$, and that there are exactly two possible different extensions for a matroid of rank~$1$.
\end{proof}

\begin{remark}
 In the bound of \eqref{eq:bndle1}, we lose a factor of up to $2^{r-1}$ from the real number. This factor is asymptotically much smaller than $\frac{2n!}{(n-r+1)!}$. In fact, it is not difficult to prove that $\lle{n}{r}\geq2^{r-1}\frac{n!}{(n-1)(n-r)!}$ by giving some cyclic order to the elements of $\cM$ and counting only the lexicographic extensions $[a_1^{s_1},\dots, a_r^{s_r}]$ that fulfill
\begin{enumerate}[(i)]
 \item For $1<i<r$, $a_i^{s_i}$ is not $b^{-\alpha s_{i-1}}$ if $b<a_{i-1}$ and $b$ and $a_{i-1}$ are $\alpha$-inseparable in $\cM/\{a_1,\dots,a_{i-2}\}$.
 \item For $1<i<r$, $a_i^{s_i}$ is not $c^{\alpha\beta s_{i-1}}$ when there exists $b$ with $c<b<a_{i-1}$ such that $b$ and $a_{i-1}$ are $\alpha$-inseparable in $\cM/\{a_1,\dots,a_{i-2}\}$ and $c$ is $\beta$-inseparable from $b$ in $\cM/\{a_1,\dots,a_{i-1}\}$.
 \item $a_r$ and $a_{r-1}$ are $\alpha$-inseparable in $\cM/\{a_1,\dots,a_{r-2}\}$, $a_{r-1}<a_r$ and $s_r=\alpha s_{r-1}$.
\end{enumerate}

 But then the formulas become more complicated and and adds nothing substantial to the result.
\end{remark}

% 
% \begin{theorem}\label{thm:lble2}
%  Let $\cM$ be a rank $r>1$ labeled oriented matroid with $n>r+1$ elements. The number of different labeled lexicographic extensions of $\cM$ fulfills \begin{equation}\lle{n}{r}\geq2^{r-1}\frac{n!}{(n-1)(n-r)!}.\end{equation}
% \end{theorem}
% \begin{proof}
% 
% There are $2^n\frac{n!}{(n-r)!}$ different signatures of lexicographic extensions, yet not all of them represent different lexicographic extensions. We aim to avoid counting the same extension twice with two different signatures. A key tool for this will be the inseparability graph.
% 
% Consider the inseparability graph $IG(\cM)$ of $\cM$, and orient it in such a way that every node has at most one outgoing edge (this is possible because of Theorem~\ref{thm:IG}). Do the same for all the inseparability graphs of contractions of $\cM$ of rank $\geq 2$, $IG(\cM/S)$.
% If $a\rightarrow b$ is a directed edge of $IG(\cM)$ then we say that $\s(a)=b$,  and say that $\alpha(a)=\alpha$ if $a$ and $b$ are $\alpha$-inseparable in $\cM$.
% 
% Let $[a_1^{s_1},\dots,a_r^{s_r}]$ and $[{a_1'}^{s_1'},\dots,{a_r'}^{s_r'}]$ be two different signatures that provide the same lexicographic extension $p$. If $a_1$ and $a_1'$ are different, then $a_1$ and $a_1'$ must be $(-s_1s_1')$-inseparable in $\cM$. Indeed, if $C$ is a cocircuit of $\cM$ with $C(a_1)\neq 0$ and $C(a_1')\neq 0$, then it extends to a cocircuit $C'$ of $\cM[p]$ with $C(a_1)=s_1C'(p)$ and $C(a_1')=s_1'C'(p)$. Analogously, if $a_i$ and $a_i'$ are different and $a_j=a_j'$ for $j<i$, then $a_i$ and $a_i'$ must be $(-s_is_i')$-inseparable in $\cM/\{a_1,\dots,a_{i-1}\}$. In general, if $a$ is $\alpha$-inseparable with $p$ in $\cM/\{a_1,\dots,a_{i-1}\}$, then $a$ and $a_i$ must be $(s_i\alpha)$-inseparable.
% 
% Still in the scenario where $a_i\neq a_i'$ and $a_j=a_j'$ for $j<i$, observe that $p$ is $(-s_i)$-inseparable with $a_i$ and $(-s_i')$-inseparable with $a_i'$ in $\cM[p]/\{a_1,\dots,a_{i-1}\}$. In particular, if we denote $S_i=\{a_1,\dots,a_{i-1},a_i\}$ then $p$ and $a_i'$ are still $(-s_i')$-inseparable in $\cM[p]/S_i=(\cM/S_i)[a_{i+1}^{s_{i+1}},\dots,a_r^{s_r}]$. As a consequence, $a_{i+1}$ and $a_i'$ must be $(-s_i' s_{i+1})$-inseparable. 
% 
% In what follows, fixed a lexicographic extension $[a_1^{s_1},\dots, a_r^{s_r}]$ of $\cM$, we define $\s_i(a)$ and $\alpha_i(a)$ as $\s(a)$ and $\alpha(a)$ in $\cM/\{a_1,\dots,a_i\}$.
% 
% 
% We define a family of lexicographic extensions $\cL$ as follows: $[a_1^{s_1},\dots, a_r^{s_r}]$ is in $\cL$ if it fulfills
% \begin{enumerate}[(i)]
%  \item For $1<i<r$, $a_i^{s_i}$ is not $\s_{i-2}(a_{i-1})^{-\alpha_{i-2}(a_{i-1})s_{i-1}}$.
%  \item For $1<i<r$, $a_i^{s_j}$ is not $\s_{i-1}(\s_{i-2}(a_{i-1}))^{\alpha_{i-1}(\s_{i-2}(a_{i-1}))\alpha_{i-2}(a_{i-1})s_{i-1} }$.
%  \item $a_r=\s_{r-2}(a_{r-1})$ and $s_r=\alpha_{r-2}(a_{r-1})s_{r-1}$.
% \end{enumerate}
% 
% We claim that there is no lexicographic extension more than once in $\cL$. In particular we will see that if a extension $p$ can be written as $[a_1^{s_1},\dots,a_{i-1}^{s_{i-1}},a_i^{s_i},\dots]$ and $[a_1^{s_1},\dots,a_{i-1}^{s_{i-1}},{a_i'}^{s_i'},\dots]$ where $a_i'=\s_{i-1}(a_i)$, and $s_i'=-\alpha_{i-1}(a_i)s_i$, then only the signature $[a_1^{s_1},\dots,a_{i-1}^{s_{i-1}},{a_i'}^{s_i'},\dots]$ can belong to $\cL$.
% 
% To prove this, we will see that in these extensions $p$ and $\s_{i-1}(a_i)$ are not $\alpha_{i-1}(a_i)s_i$ inseparable in $\cM[p]/\{a_1,\dots,a_{i}\}$. This implies our claim. Indeed, let $p$ be the extension $[a_1^{s_1},\dots,a_{i-1}^{s_{i-1}},a_i^{s_i},\dots]$, let $a_i'=\s_{i-1}(a_i)$, we want to argue that $p$ cannot also be writen as $[a_1^{s_1},\dots,a_{i-1}^{s_{i-1}},{a_i'}^{s_i'},\dots]$. If it could, then $s_i'=-\alpha_{i-1}(a_i)s_i$, and $\s_{i-1}(a_{i})$ would be $\alpha_{i-1}(a_i)s_i$ inseparable with $p$ in $\cM[p]/\{a_1,\dots,a_{i}\}$.
% 
% We prove that $p$ and $\s_{i-1}(a_i)$ are not $\alpha_{i-1}(a_i)s_i$ inseparable in $\cM[p]/\{a_1,\dots,a_{i}\}$ by induction on $r$.
% 
% First we deal with $r=2$. Let $p=[a_1^{s_1},s(a_1)^{\alpha(a_1)s_1}]$. Since $\cM[a_1^{s_1},s(a_1)^{\alpha(a_1)s_1}]/a_1=(\cM/a_1)[s(a_1)^{\alpha(a_1)s_1}]$, $p$ and $s(a_1)$ are $(-\alpha(a_1)s_1)$-inseparable in $\cM/a_1$.
% 
% For the general case, we prove that $p$ and $\s(a_1)$ are not $\alpha(a_1)s_1$ inseparable in $\cM[p]/a_1$. For $a_i$ with $i>1$, the result follows by induction using the contraction $\cM/\{a_1,\dots,a_{i-1}\}$.
% 
% If $\s(a_1)$ and $p$ are inseparable in $\cM/a_1$, then $a_2$ must be $\s(a_1)$ or inseparable with $\s(a_1)$.
% 
% If $a_2=\s(a_1)$ then, because of the restrictions on the signature, $s_2=\alpha(a_1)s_1$ and $p$ and $\s(a_1)$ are $(-\alpha(a_1)s_1)$-inseparable in $\cM/a_1$.
% 
% If $a_2=\s_1(\s(a_1))$, because of the restrictions on the signature, $s_2=-\alpha_1(\s(a_1))\alpha(a_1)s_1$, and, since $a_2$ and $\s(a_1)$ are $\alpha_1(\s(a_1))$ inseparable, the inseparability of $p$ and $\s(a_1)$ in $\cM/a_1$ can only be $$\alpha_1(\s(a_1))s_2=-\alpha_1(\s(a_1))\alpha_1(\s(a_1))\alpha(a_1)s_1=-\alpha(a_1)s_1.$$
% 
% Finally, there is the case $\s_1(a_2)=\s(a_1)$. If $p$ and $\s(a_1)$ are $(\alpha(a_1)s_1)$-inseparable in $\cM/a_1$, then $s_2=\alpha_1(a_2)\alpha(a_1)s_1$. And if $s_2=\alpha_1(a_2)\alpha(a_1)s_1$, we know by induction hypothesis that the inseparability of $p$ and $\s(a_1)$ cannot be $$\alpha_1(a_2)s_2=\alpha_1(a_2)\alpha_1(a_2)\alpha(a_1)s_1=\alpha(a_1)s_1.$$ 
% 
% This concludes the proof that there is no lexicographic extension more than once in $\cL$. It only remains to find some bound on the number of lexicographic extensions in $\cL$. For this, observe that if $1<i<r$, then $a_i$ can be any element of $\cM/\{a_1,\dots,a_{i-1}\}$ with $s_i$ any sign except for atmost two forbidden configurations (if $\s_{i-2}(a_{i-1})$ and $\s_{i-1}(\s_{i-2}(a_{i-1}))$ exist). That means that there are at least $2(n-(i-1))-2=2(n-i)$ choices, while for $a_1^{s_1}$ there are $2n$ options and $a_r^{s_r}$ is fixed. Summing up,
% $$\lle{n}{r}\geq 2n \prod_{i=2}^{r-1}2(n-i)=2^{r-1}\frac{\ffp{n}{r}}{n-1}=2^{r-1}\frac{n!}{(n-1)(n-r)!}.$$
% \end{proof}

% \subsection{The number of neighborly polytopes}

Once we have bounds for $\lle{n}{r}$, we can obtain bounds for $\lnei{n}{d}$. But first we do a case where we know the exact number.

\begin{lemma}\label{lem:nlpolygons}
 The number of labeled balanced matroids of rank $r$ with $r+3$ elements is $\frac12{(r+2)!}$.
\end{lemma}
\begin{proof}
 Balanced matroids of rank $r$ with $r+3$ elements are dual to polygons with $r+3$ vertices in $\RR^2$. There are clearly  $\frac12{(r+2)!}$ of them.
\end{proof}


We will need the following result on the inseparability graph of oriented matroids. The \defn{inseparability graph} of an oriented matroid $\cM$, $IG(\cM)$, is the graph that has the elements of $\cM$ as vertices and whose edges are the pairs of inseparable elements.
\begin{theorem}[{\cite[Theorem 1.1]{CordovilDuchet1990}}]\label{thm:IG}
 Let $\cM$ be a rank $r$ uniform oriented matroid with $n$ elements.
\begin{itemize}
 \item If $r\leq 1$ or $r\geq n-1$, then $IG ( \cM )$ is the complete graph.
 \item If $r=2$ or $r=n-2$, then $IG(\cM)$ is an $n$-cycle.
 \item If $2<r<n-2$, then $IG(\cM)$ is either a $n$-cycle, or a disjoint union of chains.
\end{itemize}
\end{theorem}

\begin{lemma}\label{lem:lbbm}
The number of labeled balanced matroids of rank $r$ with $r+1+2m$ elements fulfills 
\begin{equation*}
%\label{eq:lblneifromle}
%  \lnei{2m+r+1}{2m}\geq \prod_{i=0}^{m-1} \frac{r+2+2i}{2}\lle{r+1+2i}{r}
\lnei{2m+r+1}{2m}\geq \lnei{2m+r-1}{2m-2}\frac{r+2m}{2}\lle{r+2m-1}{r}.
\end{equation*}
\end{lemma}
\begin{proof}
 This bound is a consequence of Theorem~\ref{thm:thethm}. Fix a labeled balanced matroid~$\cM$ of rank $r$ with $r+1+2(m-1)$ elements. There are at least $\lle{r+2m-1}{r}$ different labeled lexicographic extensions on $\cM$. Let $p=[a_1^{s_1},\dots,a_r^{s_r}]$ be any such extension, and let $q$ be the extension $q=[p^-,a_1^{-},\dots,a_{r-1}^{-}]$. We count the ways of labeling $\cM[p][q]$ such that $p$ gets label $0$, and the labeling of $\cM[p][q]$ on $\cM$ preserves the relative order of the original labeling of $\cM$. There are clearly $r+2m$ ways to do it, which correspond to the possible labels that can be given to $q$. Since~$p$ is inseparable from at most two elements (see Theorem~\ref{thm:IG}), and $p$ and $q$ are inseparable, we have counted each of these labeled matroids at most twice. Which gives $\lnei{2m+r+1}{2m}\geq \lnei{2m+r-1}{2m-2}\frac{r+2m}{2}\lle{r+2m-1}{r}$.
\end{proof}

\begin{corollary}\label{cor:numbalancedfromle}
The number of labeled balanced matroids of rank $r$ with $r+1+2m$ elements fulfills 
\begin{equation*}%\label{eq:lblneifromle}
  \lnei{2m+r+1}{2m}\geq \prod_{i=0}^{m-1} \frac{r+2+2i}{2}\lle{r+1+2i}{r}.
\end{equation*}
\end{corollary}



Combining Proposition~\ref{prop:lble} and Corollary~\ref{cor:numbalancedfromle}, we get the following bound on the number of labeled balanced matroids of rank $r$ with $r+1+2m$ elements: 
\begin{equation}\label{eq:lblnei1}
 \lnei{r+1+2m}{2m}\geq\prod_{i=1}^{m} {\frac{(r+2i)!}{(2i)!}}.%\prod_{i=1}^{m} {\ffp{(r+2i)}{r}}.
\end{equation}

% 
% \begin{proposition}\label{cor:lblneibigr}
% The number of labeled neighborly polytopes in dimension $d$ with $n$ vertices fulfills 
% % \begin{equation}\label{eq:bndle2}
% %  \prod_{i=0}^{m-1} {\frac{\ffp{\left(2(r+1+2i)\right)}{2(r-1)}}{\ffp{\left(r+1+2i\right)}{(r-1)} 2^{r-2}}}
% % \end{equation}
% \begin{equation}
%  \lnei{n}{d}\geq 2^{\tfrac{d(n-d+1)}{2}\log\left(\tfrac{n-d+1}{e}\right)-\tfrac{d}{2}}.
% \end{equation}
% \end{proposition}
% \begin{proof}
% First we assume that $d=2m$ is even. Starting from Equation~\eqref{eq:lblnei1}, using that $\ffp{(r+2i)}{r}\geq \frac{(r+2)!}{2}$, 
% \begin{displaymath}
%   \lnei{r+1+2m}{2m}\geq\prod_{i=1}^{m} {\ffp{(r+2i)}{r}}\\
% 		  \geq\left(\frac{(r+2)!}{2}\right)^m
% \end{displaymath}
% If $d=2m+1$, observe that any lexicographic extension of a balanced matroid with $r+1+2m$ elements in rank $r$ will be balanced. Hence
% \begin{align*}
%   \lnei{r+2m+2}{2m+1}&\geq\lnei{r+1+2m}{2m}\ffp{(r+1+2m)}{r-1}\\&>\lnei{r+1+2m}{2m}\left(\frac{(r+2)!}{2}\right)^{\frac{1}{2}}		  \geq\left(\frac{(r+2)!}{2}\right)^{\frac{2m+1}{2}}
% \end{align*}
% 
% Now, using the inequality $k!>\left(\tfrac{k}{e}\right)^k$, and that $r+2=n-d+1$ and $m=\ffloor{d}{2}$, we get
% \begin{displaymath}
%   \lnei{n}{d}>2^{-\tfrac{d}{2}}\left(\tfrac{n-d+1}{e}\right)^{\tfrac{d(n-d+1)}{2}}=2^{\tfrac{d(n-d+1)}{2}\log\left(\tfrac{n-d+1}{e}\right)-\tfrac{d}{2}}.
% \end{displaymath}
% \end{proof}
% 
% 
% The previous bound was good when $r\gg d$, but we can do better when $r\ll d$.
% 
% \begin{proposition}\label{cor:lblneibigd}
% The number of labeled neighborly polytopes in dimension $d$ with $n$, when $d+3\leq n\leq 2d$ vertices is greater than 
% \begin{equation}
%  \lnei{n}{d}\geq 2^{\frac{(n-d-1)(d+2)}{2}\log\left(\tfrac{d+2}{e}\right)-\frac{n-d-1}{2}}
% \end{equation}
% \end{proposition}
% \begin{proof}
% First we do the case when $d=2m$ is even. Starting from Equation~\eqref{eq:lblnei1}, 
% \begin{align*}
%  \lnei{r+1+2m}{2m}&\geq\prod_{i=1}^{m}{\ffp{(r+2i)}{r}}\\
%                   &=\prod_{i=1}^{m}\prod_{j=0}^{r-1} (r+2i-j)\\
%                   &=\prod_{i=0}^{m-1}\prod_{j=1}^{r} (2m-2i+j)\\
%                   &=\prod_{i=0}^{m-1}\prod_{j=1}^{\ffloor{r}{2}} (2m-2i+2j-1)(2m-2i+2j)\prod_{i=0}^{m-1}\prod_{j=\ffloor{r}{2}+1}^{\fceil{r}{2}} (2m-2i+2j-1)\\
%                   &\geq\left(\prod_{i=0}^{m-1}(2m-2i+1)(2m-2i+2)\right)^{\ffloor{r}{2}}\prod_{j=\ffloor{r}{2}+1}^{\fceil{r}{2}}\prod_{i=0}^{m-1} (2m-2i+2)\\
% 		  &\geq\left(\frac{(2m+2)!}{2}\right)^{\ffloor{r}{2}} \prod_{j=\ffloor{r}{2}+1}^{\fceil{r}{2}}\left(\frac{(2m+2)!}{2}\right)^{\frac{1}{2}}=\left(\frac{(2m+2)!}{2}\right)^{\frac{r}{2}}
% %  		  \geq2^{-\frac{r}{2}}\left(\frac{2m+2}{e}\right)^{r(m+1)}= 2^{r(m+1)\log\left(\tfrac{2m+2}{e}\right)-\frac{r}{2}}
% \end{align*}
% For the odd case, when $d=2m+1$ (and assuming $r\geq 2$),
% \begin{align*}
%  \lnei{r+2m+2}{2m+1}&\geq\lnei{r+1+2m}{2m}\ffp{(r+1+2m)}{r-1}\\
%   &>\lnei{r+1+2m}{2m}(2m+3)^{r-1}\geq\lnei{r+1+2m}{2m}(2m+3)^{\frac{r}{2}}\\
%   &\geq\left(\frac{(2m+3)!}{2}\right)^{\frac{r}{2}}
% \end{align*}
% 
% Using the inequality $k!>\left(\tfrac{k}{e}\right)^k$, and that $r+2=n-d+1$ and $m=\ffloor{d}{2}$, we get
% \begin{align*} 
% \lnei{n}{d}&\geq\left(\frac{(d+2)!}{2}\right)^{\frac{n-d-1}{2}}
% \geq2^{\frac{-(n-d-1)}{2}}\left(\frac{d+2}{e}\right)^{\frac{(n-d-1)(d+2)}{2}}\\&= 2^{\frac{(n-d-1)(d+2)}{2}\log\left(\tfrac{d+2}{e}\right)-\frac{n-d-1}{2}}
% \end{align*}
% \end{proof}
% % \ojo{Can be done using Stirling and $(2n-1)!!=\frac{(2n)!}{2^nn!}\sim\left(\frac{2n}{e}\right)^n\sqrt{2}$, we get rid of the floor}

% It is easy to get better bounds for the number of neighborly polytopes using approximations of sums by integrals.

\begin{theorem}\label{thm:lblnei}
The number of labeled neighborly polytopes in dimension $d$ with $n$ vertices fulfills 
\begin{equation*}
\lnei{r+d+1}{d}\geq \frac{\left( r+d \right) ^{\left( \frac{r}{2}+\frac{d}{2} \right) ^{2}}}{{r}^{{(\frac{r}{2})}^{2}}{d}^{{(\frac{d}{2})}^{2}}{\e^{3\frac{r}{2}\frac{d}{2}}}},
\end{equation*}
that is, 
\begin{equation*}
 \lnei{n}{d}\geq \frac{\left(n-1\right) ^{\left( \frac{n-1}{2}\right) ^{2}}}{{(n-d-1)}^{{\left(\frac{n-d-1}{2}\right)}^{2}} d  ^{{(\frac{d}{2})}^{2}}{\e^{\frac{3d(n-d-1)}{4}}}}.
\end{equation*}
\end{theorem}
\begin{proof}
First we assume that $d=2m$ is even. We start from Equation~\eqref{eq:lblnei1}, and try to approximate the natural logarithm of $\lnei{r+1+2m}{2m}$. Using that for any increasing function $f$, $\int_{s=a-1}^{b} f(s)\  \mathrm{d}s \le \sum_{i=a}^{b} f(i)$, we get 
% $\le \int_{s=a}^{b+1} f(s)\ ds$. 
\begin{align*}
\ln\left( \lnei{r+1+2m}{2m}\right)\geq& \ln\left(\prod_{i=1}^{m} {\ffp{(r+2i)}{r}}\right)=\sum_{i=1}^{m} {\sum_{j=0}^{r-1}{ \ln\left(r+2i-j\right)}}\\
=&\sum_{i=1}^{m} {\sum_{j=1}^{r}{ \ln\left(2i+j\right)}}\geq\int_{i=0}^{m} {\int_{j=0}^{r}{ \ln\left(2i+j\right) \mathrm{d}j} \mathrm{d}i}\\
% =&  \frac{\left( 2m+r \right) ^{2}\ln  \left( 2\,m+r
%  \right)}{4}-\frac{{r}^{2}\ln  \left( r \right)}{4} -{m}^{2} \ln  \left( 2m
%  \right) -\frac{3mr}{2}.
=&  \frac{\left( 2m+r \right) ^{2}\ln  \left( 2\,m+r
 \right)-{r}^{2}\ln  \left( r \right)}{4} -{m}^{2} \ln  \left( 2m
 \right) -\frac{3mr}{2}.
\end{align*}

Hence,
\begin{align*}
\lnei{r+1+2m}{2m}\geq&\frac{\left( 2\,m+r
 \right) ^{\frac14 \left( 2\,m+r \right) ^{2}}}{{r}^{\frac14{r}^{2}}\left( 2\,m \right) ^{{m}^{2}}{\e^{\frac32mr}}}.
% \\
% =&{r}^{-1/4\,{r}^{2}} \left( 2\,m \right) ^{-{m}^{2}} \left( 2\,m+r  \right) ^{1/4\, \left( 2\,m+r \right) ^{2}}{\e^{-3/2\,mr}}
\end{align*}
And therefore,
% \begin{equation}\label{eq:lblnei}
% \lnei{n}{d}\geq\frac{\left(n-1\right) ^{\left( \frac{n-1}{2}\right) ^{2}}}{{(n-d-1)}^{{\left(\frac{n-d-1}{2}\right)}^{2}} d  ^{{(\frac{d}{2})}^{2}}{\e^{\frac{3d(n-d-1)}{4}}}}.
% \end{equation}
\begin{equation}\label{eq:lblnei}
\lnei{r+d+1}{d}\geq \frac{\left( r+d \right) ^{\left( \frac{r}{2}+\frac{d}{2} \right) ^{2}}}{{r}^{{(\frac{r}{2})}^{2}}{d}^{{(\frac{d}{2})}^{2}}{\e^{3\frac{r}{2}\frac{d}{2}}}}.
% \frac{\left(n-1\right) ^{\left( \frac{n-1}{2}\right) ^{2}}}{{(n-d-1)}^{{\left(\frac{n-d-1}{2}\right)}^{2}} d  ^{{(\frac{d}{2})}^{2}}{\e^{\frac{3d(n-d-1)}{4}}}}.
\end{equation}
 
If $d=2m+1$, observe that any lexicographic extension of a balanced matroid with $r+1+2m$ elements in rank $r$ will be balanced. Moreover, if this extension is of the form $p=[a_1^+,\dots]$ (like the extensions in Proposition~\ref{prop:lble}), then $p$ and $a_1$ are the only pair of contravariant elements in $\cM$. Hence we can assign any of the possible $r+2m+2$ labels to $p$ and we will have counted the extension at most twice.
Therefore,

\begin{align*}
  \lnei{r+2+2m}{2m+1}&\geq\lnei{r+1+2m}{2m}\frac{2r+2m+2}{2}\lle{r+1+2m}{r}\\
% 		     &\geq\lnei{r+1+2m}{2m}\frac{2r+2m+2}{2}2\prod_{j=0}^{r-1}{(r+1+2m-j)}\\
% 		     &\geq\lnei{r+1+2m}{2m}({2r+2m+2})\prod_{j=0}^{r-1}{(r+1+2m-j)}\\
 &\geq\lnei{r+1+2m}{2m}\prod_{j=0}^{r}{(2+2m+j)}
% 		      &=\lnei{r+1+2m}{2m}\prod_{j=0}^{r}{(2+2m+j)}
\end{align*}
Now,
\begin{align*}
%   \ln(\lnei{r+2m+2}{2m+1})&\geq \int_{j=0}^{r} {\int_{i=0}^{m}{ \ln\left(2i+j\right) \mathrm{d}i}\mathrm{d}j}
%  +\int_{j=-1}^{r}{ \ln\left(2m+2+j\right) \mathrm{d}j} \\
 \ln(\lnei{r+2m+2}{2m+1})&\geq \int_{j=0}^{r} {\int_{i=0}^{m}{ \ln\left(2i+j\right) \mathrm{d}i}\mathrm{d}j}
 +\int_{j=0}^{r}{ \ln\left(2m+2+j\right) \mathrm{d}j} \\
  &\geq \int_{j=0}^{r} {\int_{i=0}^{m+\frac{1}{2}}{ \ln\left(2i+j\right) \mathrm{d}i}\mathrm{d}j}.
\end{align*}
This last inequality is due to $\ln\left(2m+2+j\right)\geq \int_{i=m}^{m+\frac{1}{2}}{ \ln\left(2i+j\right) \mathrm{d}i}$ and proves that Equation~\eqref{eq:lblnei} also holds for odd dimension.
\end{proof}

\begin{corollary}
If $n>2d$, the number of labeled neighborly polytopes in dimension $d$ with $n$ vertices fulfills 
\begin{equation*}
 \lnei{n}{d}\geq \left(\frac{n-1}{\sqrt{\e^{3}}}\right)^{\frac{d(n-1)}{2}}.
\end{equation*}
\end{corollary}



